J-PAS: unprecedented precision in stellar populations of diffuse tidal features

Galaxies frequently interact with nearby systems, a process that can significantly alter their morphology and star formation activity. However, spectroscopic studies of their faint and diffuse remnants require very long exposure times and often exceed the limited field of view of integral field units (IFUs). On the other hand, broad-band imaging can have a much wider field of view, but lacks the spectral resolution to identify key spectral features, restricting accurate constraints on stellar population properties. With its 54 narrow-band filters in the optical and wide coverage (planned 8000 square degrees), J-PAS fills this gap. In this case study, we examine PGC 3087775, a massive galaxy at z = 0.046179 (~ 201 Mpc) in the later stages of a major merger in the J-PAS early data release. Photometry was validated with MaNGA IFU data (for the central part). Stellar population properties was derived using both J-PAS and SDSS photometry. SDSS indicates a metal-rich population with an extended star formation history (SFH) and elevated star formation rates. J-PAS instead points to a less metal-rich population with moderate extinction and a more rapid SFH, consistent with a quenched stellar population. The average Dn(4000) index of the tidal features is 1.24, suggesting that it was a non-dry merger and a fourfold improvement in the precision of stellar mass and Dn (4000) was found with J-PAS. We also assessed two heuristic methods for estimating the mass-to-light ratio from SDSS filters and found that they overestimate the stellar mass in this galaxy by 0.5 dex and 0.4 dex relative to SED fitting results from J-PAS and SDSS, respectively. Future work will extend this analysis to a larger sample of merging galaxies and evolution of the stellar populations of such structures across the nearby Universe to unprecedented detail. This project is fully reproducible, through Maneage (commit 0f0d7e2).

==> project <==
#!/bin/sh
#
# High-level script to manage the project.
# Run './project --help' for a description of how to use it.
#
# Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
# Copyright (C) 2021-2025 Raul Infante-Sainz <infantesainz@gmail.com>
#
# This program is free software: you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation, either version 3 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program.  If not, see <http://www.gnu.org/licenses/>.


# Basic settings
# --------------
# Stop the script if there are any errors.
set -e





# Default option values
jobs=0     # 0 is for the default for the 'configure.sh' script.
group=
debug=
quiet=0
timing=0
host_cc=0
offline=
operation=
build_dir=
input_dir=
keep_going=
check_config=
make_targets=
software_dir=
pauseformsg=1
clean_texdir=0
prepare_redo=0
highlightnew=0
all_highlevel=0
existing_conf=0
highlightnotes=0
scriptname="./project"





# Parse the options
# -----------------
#
# Separate command-line arguments from options. Then put the option value
# into the respective variable.
#
# Each option has two lines because we want to process both these formats:
# '--name=value' and '--name value'. The former (with '=') is a single
# command-line argument, so we just need to shift the counter by one. The
# latter (without '=') is two arguments, so we'll need two shifts.
#
# Note on the case strings: for every option, we need three lines: one when
# the option name and value are separate. Another when there is an equal
# between them, and finally one where the value is immediately after the
# short-format. This exact order is important. Otherwise, there will be a
# conflict between them.

print_help() {
    # Print the output.
    cat <<EOF
Usage: $scriptname configure [OPTIONS]
       $scriptname shell     [OPTIONS]
       $scriptname make      [OPTIONS]

Top-level script to manage the reproducible project. The high-level
operation is defined by the (mandatory) second argument:

  configure    - Configure project for this machine (e.g., build software).
  make         - Run the project (do analysis and build outputs).
  shell        - Execute the project's shell for interactive testing.

RECOMMENDATION: If this is the first time you are configuring this
template, please don't use the options and let the script explain each
parameter in full detail by simply running './project configure'.

Project 'make' special tagets
  ./project make           Build the project on one thread
  ./project make -jN       Built the project in parallel on N threads.
  ./project make clean     Clean all files generated by 'make' (not software).
  ./project make texclean  Clean all files built by (La)TeX.
  ./project make distclean Clean everything (including compiled software).
  ./project make dist      Produce a LaTeX-ready-to-build distribution tarball
                           ('tar.gz') of the project. This is ready to be
                           uploaded to servers like 'arXiv.org'.
  ./project make dist-lzip Similar to 'dist', but compress to '.tar.lz'.
  ./project make dist-zip  Similar to 'dist', but compress to '.zip'.
  ./project make dist-software  Build a .tar.gz tarball containing all
                                software source tarballs necessary for the
                                project.

With the options below you can modify the default behavior.
Configure options:
      --all-highlevel      Build all high-level software (for development).
  -b, --build-dir=STR      Top directory to build the project in.
      --check-config       During configuration, show what is being built.
      --clean-texdir       Remove possibly existing build-time subdirectories
                           under the project's 'tex/' directory (can happen
                           when source is from arXiv for example).
  -e, --existing-conf      Use (possibly existing) local configuration.
  -i, --input-dir=STR      Directory containing input datasets (optional).
      --host-cc            Use host system's C compiler, don't build GCC.
      --quiet              Do not print basic info messages (with '-e').
      --no-pause           Do not sleep/pause after basic info messages.
  -s, --software-dir=STR   Directory containing necessary software tarballs.

Configure and Make options:
  -d, --debug[=FLAGS]      In configure: use -j1, no -k, and no Zenodo check.
                           In make: 'FLAGS' will be directly passed to 'make'.
  -k, --keep-going         Keep going when some targets can't be made.
  -g, --group=STR          Build and run with write permissions for a group.
  -j, --jobs=INT           Number of threads to build/run the software.
  -?, --help               Print this help list.

Make (analysis) options:
  -p, --prepare-redo       Re-do preparation (only done automatically once).
  -t, --timing             Starting and ending times written in 'timing.txt'.

Make (final PDF) options:
      --refresh-bib        Force refresh the bibliography.
      --highlight-all      Activate '--highlight-new' & '--highlight-notes'.
      --highlight-new      Highlight '\new' parts of text as green.
      --highlight-notes    Show '\tonote' regions as red text in PDF.

Mandatory or optional arguments to long options are also mandatory or optional
for any corresponding short options.

Maneage URL: https://maneage.org

Report bugs to mohammad@akhlaghi.org
EOF
}

on_off_option_error() {
    if [ "x$2" = x ]; then
        echo "$scriptname: '$1' doesn't take any values."
    else
        echo "$scriptname: '$1' (or '$2') doesn't take any values."
    fi
    exit 1
}

check_v() {
    if [ x"$2" = x ]; then
        echo "$scriptname: option '$1' requires an argument."
        echo "Try '$scriptname --help' for more information."
        exit 1;
    fi
}

func_operation_set() {
    if [ x$operation = x ]; then
        operation=$1
    else
        echo "Only one operation ('configure', 'make' or 'shell') may be given."
        exit 1
    fi
}

while [ $# -gt 0 ]
do
 case $1 in
  # Main operation.
  configure)    func_operation_set $1; shift;;
  make)         func_operation_set $1; shift;;
  shell)        func_operation_set $1; shift;;

  # Configure options:
  -e|--existing-conf)    existing_conf=1;                                                          shift;;
  -e*|--existing-conf=*) on_off_option_error --existing-conf -e;;
  --host-cc)             host_cc=1;                                                                shift;;
  --host-cc=*)           on_off_option_error --host-cc;;
  --offline)             offline=1;                                                                shift;;
  --offline=*)           on_off_option_error --offline;;
  -i|--input-dir)        input_dir="$2";                             check_v "$1" "$input_dir";    shift;shift;;
  -i=*|--input-dir=*)    input_dir="${1#*=}";                        check_v "$1" "$input_dir";    shift;;
  -i*)                   input_dir=$(echo    "$1" | sed -e's/-i//'); check_v "$1" "$input_dir";    shift;;
  -s|--software-dir)     software_dir="$2";                          check_v "$1" "$software_dir"; shift;shift;;
  -s=*|--software-dir=*) software_dir="${1#*=}";                     check_v "$1" "$software_dir"; shift;;
  -s*)                   software_dir=$(echo "$1" | sed -e's/-s//'); check_v "$1" "$software_dir"; shift;;
  --check-config)        check_config=1;                                                           shift;;
  --check-config=*)      on_off_option_error --check-config;;
  --clean-texdir)        clean_texdir=1;                                                           shift;;
  --clean-texdir=*)      on_off_option_error --clean-texdir;;
  --all-highlevel)       all_highlevel=1;                                                          shift;;
  --all-highlevel=*)     on_off_option_error --all-highlevel;;
  --no-pause)            pauseformsg=0;                                                            shift;;
  --no-pause=*)          on_off_option_error --no-pause;;
  --quiet)               quiet=1;                                                                  shift;;
  --quiet=*)             on_off_option_error --quiet;;

  # Configure and Make options:
  -b|--build-dir)        build_dir="$2";                             check_v "$1" "$build_dir";shift;shift;;
  -b=*|--build-dir=*)    build_dir="${1#*=}";                        check_v "$1" "$build_dir";shift;;
  -b*)                   build_dir=$(echo    "$1" | sed -e's/-b//'); check_v "$1" "$build_dir";shift;;
  -g|--group)            group="$2";                                 check_v group "$group";   shift;shift;;
  -g=*|--group=*)        group="${1#*=}";                            check_v group "$group";   shift;;
  -g*)                   group=$(echo   "$1" | sed -e's/-g//');      check_v group "$group";   shift;;
  -j|--jobs)             jobs="$2";                                  check_v jobs  "$jobs";    shift;shift;;
  -j=*|--jobs=*)         jobs="${1#*=}";                             check_v jobs  "$jobs";    shift;;
  -j*)                   jobs=$(echo "$1" | sed -e's/-j//');         check_v jobs  "$jobs";    shift;;
  -k|--keep-going)       keep_going="--keep-going";                                            shift;;
  -k=*|--keep-going=*)   on_off_option_error --keep-going -k;;
  -k*)                   on_off_option_error --keep-going -k;;
  -'?'|--help)           print_help; exit 0;;
  -'?'*|--help=*)        on_off_option_error --help -?;;

  # Make options (analysis):
  -p|--prepare-redo)     prepare_redo=1;                                                  shift;;
  -p=*|--prepare-redo=*) on_off_option_error --prepare-redo;                              shift;;
  -t|--timing)           timing=1;                                                        shift;;
  -t=*|--timing=*)       on_off_option_error --timing;                                    shift;;

  # Make options (final PDF):
  --refresh-bib)         [ -f tex/src/references.tex ] && touch tex/src/references.tex;   shift;;
  --highlight-all)       highlightnew=1; highlightnotes=1;                                shift;;
  --highlight-all=*)     on_off_option_error --highlight-new;;
  --highlight-new)       highlightnew=1;                                                  shift;;
  --highlight-new=*)     on_off_option_error --highlight-new;;
  --highlight-notes)     highlightnotes=1;                                                shift;;
  --highlight-notes=*)   on_off_option_error --highlight-notes;;
  -d|--debug)            if [ x$operation = x ]; then
                             echo "Please set the operation before calling '--debug'"; exit 1
                         elif [ x$operation = xconfigure ]; then debug=a;   shift;
                         elif [ x$operation = xmake ]; then
                             if [ x"$2" = x ]; then
                                 echo "In make-mode, '--debug' needs a value; see GNU Make manual"; exit 1
                             else debug="$2"; check_v debug "$debug"; shift;shift; fi
                         else
                             echo "Operation '$operation' not recognized, please use 'configure' or 'make'"
                         fi;;
  -d=*|--debug=*)        debug="${1#*=}";                       check_v debug "$debug";   shift;;
  -d*)                   debug=$(echo "$1" | sed -e's/-d//');   check_v debug "$debug";   shift;;

  # Unrecognized option:
  -*) echo "$scriptname: unknown option '$1'"; exit 1;;

  # Not an option, an argument (so its a Make target).
  *) make_targets="$make_targets $1"; shift;;
 esac
done





# Check configuration status
# --------------------------
if ! [ x$check_config = x ]; then
    # Find the color option to pass to 'ls'. Note that '--color' (for GNU
    # Coreutils 'ls') should be checked first because it also has '-G', but
    # for something else.
    if   ls --color 2> /dev/null > /dev/null; then coloropt="--color=auto"
    elif ls -G      2> /dev/null > /dev/null; then coloropt="-G"
    else                               coloropt=""
    fi

    # Print a notice to let the user know what is happening.
    cat <<EOF

This is an infinite loop that will print what software are being built at
every moment. It is actually a listing ('ls' command) of the temporary
directory where software source code are unpacked while they are being
built. If the project isn't being configured, the output (every second)
will either be empty (only a date) or a with an error about a non-existant
directory. This feature is thus only useful when the project's software are
being built.

EOF

    # Run the infinite loop. To be able to find the last built programs, we
    # need to put all the Python programs and high-level program into one
    # directory.
    checkdir=.local/version-info/.for-check-config
    while true; do

        # Make sure the '.build' directory has already been created.
        echo;
        echo "========================"
        if [ -d .build ]; then
            echo "$(date)    [[press CTRL-C to stop]]";
            echo "--- Currently being built:"
            if [ -d .build/software/build-tmp ]; then
                ls $coloropt .build/software/build-tmp || junk=1;
            fi

            # Make the temporary directory, delete its contents, then put
            # new links of all built software.
            if ! [ -d $checkdir ]; then mkdir $checkdir; fi
            rm -f $checkdir/*

            # Check if any programs exist in the given directory yet.
            printresults=0
            check=$(ls .local/version-info/python/)
            if ! [ "x$check" = x ]; then
                printresults=1
                ln -s "$(pwd)"/.local/version-info/python/*  $checkdir/
            fi
            check=$(ls .local/version-info/proglib/)
            if ! [ "x$check" = x ]; then
                printresults=1
                ln -s "$(pwd)"/.local/version-info/proglib/* $checkdir/
            fi

            # If something was actually found, then print them.
            if [ $printresults = 1 ]; then
                echo "--- Last 5 packages that were built:"

                # Then sort all the links based on the most recent dates of
                # the files they link to (with '-L').
                ls -Llt $checkdir  \
                    | awk '/^-/ && c++<5 {printf "[at %s] %s\n", \
                                                 $(NF-1), $NF}'
            fi
        else
            cat <<EOF
The connection to the build directory (.build) is not yet created.

If you have just ran './project configure', it should be created and will
be used in a few seconds to report the build status of various software.
If not, please run './project configure' (in another terminal) and you will
see the results shortly afterwards.
EOF
        fi
        echo "========================"

        # Wait for the next round of checks.
        sleep 1
    done
    exit 0
fi





# Group check
# -----------
if ! [ x$group = x ]; then

    # Check if group is usable.
    if ! sg "$group" "echo Group \'$group\' exists"; then
        printf "$scriptname: '$group' is not a usable group name on "
        printf "this system. TIP: you can use the 'groups' command "
        printf "to see your groups)\n"
        exit 1
    fi

    # Set the group option for running Make.
    gopt="maneage_group_name=$group"
fi





# Build directory symbolic links
# ------------------------------
#
# The source directory will contain two symbolic links that point to the
# build directory:

#   - .build: the top build directory.
#
#   - .local: the second to the top software installed directory. They are
#     used during the configuration phase to simplify commands and are also
#     very useful during the development of a maneage'd project (to easily
#     get to the build directory or execut Maneage'd software).
#
# This needs to be done on every run because:
#   - './project configure' can be run with a new build directory, and
#     keeping the old '.build' conflicts with the new build directory
#     that the user gave.
#   - './project make' or './project shell' (within a newly cloned source
#     directory from inside a container): the links do not exist but have
#     to be set to the container's build directory.
#   - This is not an expensive operation.
if ! [ x"$build_dir" = x ]; then
    rm -f .build .local
    ln -s $build_dir .build
    ln -s $build_dir/software/installed .local
fi





# Function to validate configuration
# ----------------------------------
#
# Check if the configuration is missing/incomplete
configuration_check() {
    confdone=software/config/hardware-parameters.tex
    if ! [ -f .build/$confdone ]; then
        cat <<EOF

The project is either (1) not configured on this system, or (2) the
configuration wasn't successful.

(1) If it hasn't been configured at all, use the command below to configure
it (set a build directory and let it build its necessary software in it).

      $ ./project configure

(2) If it has been configured, but the configuration failed in a step, you
can re-configure it using your previous settings with the command
below. All successful steps will be skipped, allowing a fast completion.

      $ ./project configure -e

If there was a problem, please let us know by filling this online form:
      http://savannah.nongnu.org/support/?func=additem&group=reproduce

EOF
        exit 1
    fi
}





# Function for TeX Preparations
# -----------------------------
#
# Make sure that the necessary analysis directories directory exist in the
# build directory. These will be necessary in various phases of hte
# analysis and having them inside the lower-level Make steps will require
# setting them as prerequisites for many basic jobs (thus making the
# Makefiles harder to read and add potentials for bugs: forgetting to add
# them for example). Also, we don't want the configure phase to make any
# edits in the analysis directory, so they are not built there.
tex_preparations () {

    # Extract the location of the build directory.
    bdir=$(.local/bin/realpath .build)

    # We are using our custom-built 'mkdir' which is guaranteed to have the
    # '-p' option (that will also build intermediate directories) and won't
    # complain if the directory already exists.
    badir=$bdir/analysis
    texdir=$badir/tex
    btexdir=$texdir/build
    tikzdir=$btexdir/tikz
    mtexdir=$texdir/macros
    .local/bin/mkdir -p $mtexdir $btexdir $tikzdir

    # If 'tex/build' and 'tex/tikz' are symbolic links then 'rm -f'
    # will delete them and we can continue. However, when the project
    # is being built from the tarball (from arXiv for example), these
    # two are not symbolic links but actual directories with the
    # necessary built-components to build the PDF in them. In this
    # case, because 'tex/build' is a directory, 'rm -f' will fail, so
    # we'll just rename the two directories (as backup) and let the
    # project build the proper symbolic links afterwards.
    if rm -f tex/build; then
        rm -f tex/tikz
    else
        mv tex/tikz  tex/tikz-from-tarball
        mv tex/build tex/build-from-tarball
    fi

    # Build the symbolic links.
    if ! [ -L tex/tikz ]; then ln -s "$tikzdir" tex/tikz; fi
    if ! [ -L tex/build ]; then ln -s "$texdir" tex/build; fi
}





# Function to run in controlled environment
# -----------------------------------------
#
# Controlling the environment is necessary for running the analysis. Like
# the other funcitons here, this is defined to simplify the high-level code
# within the 'make)' switch statement.
perms="u+r,u+w,g+r,g+w,o-r,o-w,o-x"
controlled_env() {

    # Get the full address of the build directory:
    bdir=`.local/bin/realpath .build`

    # Remove all existing environment variables (with 'env -i') and only
    # use some pre-defined environment variables, then build the project.
    envmake=".local/bin/env -i HOME=$bdir sys_rm=$(which rm) $gopt"
    envmake="$envmake highlightnew=$highlightnew"
    envmake="$envmake highlightnotes=$highlightnotes .local/bin/make"
    envmake="$envmake --no-builtin-rules --no-builtin-variables -f $1"
    envmake="$envmake $keep_going"
    if ! [ x"$debug" = x  ]; then envmake="$envmake --debug=$debug"; fi

    # Set the number of jobs. Note that for the 'configure.sh' script the
    # default value has to be 0, so the default is the maximum number of
    # threads. But here, the default value is 1.
    if ! [ x"$jobs"  = x0 ]; then envmake="$envmake -j$jobs";  fi

    # Run the project
    if [ x"$group" = x ]; then
        $envmake $make_targets
    else
        # Set the group and permission flags.
        sg "$group" "umask $perms && $envmake $make_targets"
    fi
}





# Do requested operation
# ----------------------
configscript=./reproduce/software/shell/configure.sh
case $operation in

    # Build the project's software.
    configure)

        # Set executable flags
        # --------------------
        #
        # In some scenarios (for example when using a tarball from arXiv),
        # it may happen that the host server has removed the executable
        # flags of all the files. In 'README.md' we instruct the readers on
        # setting the executable flag of this script. But we don't want the
        # user to have to worry about any other file that needs an
        # executable flag.
        #
        # Basically, all the project shell scripts need executable flags so
        # to make sure they have them, we are activating the executable
        # flags by default here every time './project configure' is run. If
        # any other file in your project needs such flags, add them here.
        if ! [ -x reproduce/software/shell/configure.sh ]; then
            chmod +x reproduce/analysis/bash/* \
                     reproduce/software/shell/* \
                     reproduce/software/config/*.sh
        fi

        # If the user requested, clean the TeX directory from the extra
        # (to-be-built) directories that may already be there (and will not
        # allow the configuration to complete).
        if [ x"$clean_texdir" = x1 ]; then
            rm -rf tex/build tex/tikz
        fi

        # Variables to pass to the configuration script.
        export jobs=$jobs
        export debug=$debug
        export quiet=$quiet
        export host_cc=$host_cc
        export offline=$offline
        export build_dir=$build_dir
        export input_dir=$input_dir
        export scriptname=$scriptname
        export pauseformsg=$pauseformsg
        export maneage_group_name=$group
        export software_dir=$software_dir
        export existing_conf=$existing_conf
        export all_highlevel=$all_highlevel

        # Run the configuration script
        if [ x"$group" = x ]; then
            $configscript
        else
            # Set the group and permission flags.
            sg "$group" "umask $perms && $configscript"

            # Set the group writing permission for everything in the
            # installed software directory. The common build process sets
            # the writing permissions of the installed programs/libraries
            # to '755'. So group members can't write over a file. This
            # creates problems when another group member wants to update
            # the software for example. We thus need to manually add the
            # group writing flag to all installed software files.
            printf "Enabling group writing permission on all installed "
            printf "software...\n"
            .local/bin/chmod -R g+w .local/;
        fi
        ;;





    # Batch execution of the project.
    make)

        # Make sure the configure script is complete and necessary LaTeX
        # directories are in place.
        configuration_check
        tex_preparations

        # Register the start of this run if requested (we are appending the
        # new information so previous information is preserved until the
        # user intentionally deletes/cleans it).
        if [ $timing = 1 ]; then echo "start: $(date)" >> timing.txt; fi

        # Run data preparation phase (optionally build Makefiles with
        # special values for optimizing the main 'top-make.mk'). But note
        # that data preparation is only done automatically the first time
        # the project is built (when '.build/analysis/preparation-done.mk'
        # doesn't yet exist). After that, if the user wants to re-do the
        # preparation they have to use the '--prepare-redo' option.
        if ! [ -f .build/analysis/preparation-done.mk ] \
                || [ x"$prepare_redo" = x1 ]; then
            controlled_env reproduce/analysis/make/top-prepare.mk
        fi

        # Call top-make (highest level analysis Makefile).
        controlled_env reproduce/analysis/make/top-make.mk

        # Register the time of the project's ending.
        if [ $timing = 1 ]; then echo "end:   $(date)" >> timing.txt; fi
        ;;





    # Interactive shell of Maneage.
    shell)

        # Make sure the configure script has been completed properly.
        configuration_check

        # Run the project's own shell without inheriting any environment
        # from the host. The 'TERM' environment variable is necessary for
        # tools like some text editors.
        bdir=$(.local/bin/realpath .build)
        instdir="$bdir"/software/installed
        bindir="$bdir"/software/installed/bin
        rcfile=$(pwd)/reproduce/software/shell/bashrc.sh
        .local/bin/env -i \
            HOME="$bdir" \
            TERM="$TERM" \
            PATH="$bindir" \
            CCACHE_DISABLE=1 \
            PROJECT_STATUS=shell \
            SHELL="$bindir"/bash \
            COLORTERM="$COLORTERM" \
            PROJECT_RCFILE="$rcfile" \
            LDFLAGS=-L"$instdir"/lib \
            CPPFLAGS=-I"$instdir"/include \
            LD_LIBRARY_PATH="$instdir"/lib \
            OMPI_MCA_plm_rsh_agent=/bin/false \
            PYTHONPATH="$instdir"/lib/python/site-packages \
            PYTHONPATH3="$instdir"/lib/python/site-packages \
            PS1="[\[\033[01;35m\]maneage@\h \W\[\033[32m\]\[\033[00m\]]$ " \
            "$bindir"/bash --noprofile --rcfile "$rcfile"
        ;;





    # Operation not specified.
    *)
        cat <<EOF

No operation defined!

Please run with '--help' for more information.
(TIP: available operations are: 'configure', 'make', or 'shell').

EOF
        exit 1
        ;;
esac


==> reproduce/software/bibtex/astrometrynet.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{astrometrynet,
       author = {{Lang}, Dustin and {Hogg}, David W. and {Mierle}, Keir and {Blanton}, Michael and {Roweis}, Sam},
        title = "{Astrometry.net: Blind Astrometric Calibration of Arbitrary Astronomical Images}",
      journal = {AJ},
     keywords = {astrometry, catalogs, instrumentation: miscellaneous, methods: data analysis, methods: statistical, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2010,
        month = may,
       volume = {139},
       number = {5},
        pages = {1782-1800},
          doi = {10.1088/0004-6256/139/5/1782},
archivePrefix = {arXiv},
       eprint = {0910.2233},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010AJ....139.1782L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/astropy.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{astropy2018,
   author = {{Astropy Collaboration} and {Price-Whelan}, A.~M. and {Sip{\H o}cz}, B.~M. and
	{G{\"u}nther}, H.~M. and {Lim}, P.~L. and {Crawford}, S.~M. and
	{Conseil}, S. and {Shupe}, D.~L. and {Craig}, M.~W. and {Dencheva}, N. and
	{Ginsburg}, A. and {VanderPlas}, J.~T. and {Bradley}, L.~D. and
	{P{\'e}rez-Su{\'a}rez}, D. and {de Val-Borro}, M. and {Aldcroft}, T.~L. and
	{Cruz}, K.~L. and {Robitaille}, T.~P. and {Tollerud}, E.~J. and
	{Ardelean}, C. and {Babej}, T. and {Bach}, Y.~P. and {Bachetti}, M. and
	{Bakanov}, A.~V. and {Bamford}, S.~P. and {Barentsen}, G. and
	{Barmby}, P. and {Baumbach}, A. and {Berry}, K.~L. and {Biscani}, F. and
	{Boquien}, M. and {Bostroem}, K.~A. and {Bouma}, L.~G. and {Brammer}, G.~B. and
	{Bray}, E.~M. and {Breytenbach}, H. and {Buddelmeijer}, H. and
	{Burke}, D.~J. and {Calderone}, G. and {Cano Rodr{\'{\i}}guez}, J.~L. and
	{Cara}, M. and {Cardoso}, J.~V.~M. and {Cheedella}, S. and {Copin}, Y. and
	{Corrales}, L. and {Crichton}, D. and {D'Avella}, D. and {Deil}, C. and
	{Depagne}, {\'E}. and {Dietrich}, J.~P. and {Donath}, A. and
	{Droettboom}, M. and {Earl}, N. and {Erben}, T. and {Fabbro}, S. and
	{Ferreira}, L.~A. and {Finethy}, T. and {Fox}, R.~T. and {Garrison}, L.~H. and
	{Gibbons}, S.~L.~J. and {Goldstein}, D.~A. and {Gommers}, R. and
	{Greco}, J.~P. and {Greenfield}, P. and {Groener}, A.~M. and
	{Grollier}, F. and {Hagen}, A. and {Hirst}, P. and {Homeier}, D. and
	{Horton}, A.~J. and {Hosseinzadeh}, G. and {Hu}, L. and {Hunkeler}, J.~S. and
	{Ivezi{\'c}}, {\v Z}. and {Jain}, A. and {Jenness}, T. and {Kanarek}, G. and
	{Kendrew}, S. and {Kern}, N.~S. and {Kerzendorf}, W.~E. and
	{Khvalko}, A. and {King}, J. and {Kirkby}, D. and {Kulkarni}, A.~M. and
	{Kumar}, A. and {Lee}, A. and {Lenz}, D. and {Littlefair}, S.~P. and
	{Ma}, Z. and {Macleod}, D.~M. and {Mastropietro}, M. and {McCully}, C. and
	{Montagnac}, S. and {Morris}, B.~M. and {Mueller}, M. and {Mumford}, S.~J. and
	{Muna}, D. and {Murphy}, N.~A. and {Nelson}, S. and {Nguyen}, G.~H. and
	{Ninan}, J.~P. and {N{\"o}the}, M. and {Ogaz}, S. and {Oh}, S. and
	{Parejko}, J.~K. and {Parley}, N. and {Pascual}, S. and {Patil}, R. and
	{Patil}, A.~A. and {Plunkett}, A.~L. and {Prochaska}, J.~X. and
	{Rastogi}, T. and {Reddy Janga}, V. and {Sabater}, J. and {Sakurikar}, P. and
	{Seifert}, M. and {Sherbert}, L.~E. and {Sherwood-Taylor}, H. and
	{Shih}, A.~Y. and {Sick}, J. and {Silbiger}, M.~T. and {Singanamalla}, S. and
	{Singer}, L.~P. and {Sladen}, P.~H. and {Sooley}, K.~A. and
	{Sornarajah}, S. and {Streicher}, O. and {Teuben}, P. and {Thomas}, S.~W. and
	{Tremblay}, G.~R. and {Turner}, J.~E.~H. and {Terr{\'o}n}, V. and
	{van Kerkwijk}, M.~H. and {de la Vega}, A. and {Watkins}, L.~L. and
	{Weaver}, B.~A. and {Whitmore}, J.~B. and {Woillez}, J. and
	{Zabalza}, V. and {Astropy Contributors}},
    title = "{The Astropy Project: Building an Open-science Project and Status of the v2.0 Core Package}",
  journal = {AJ},
archivePrefix = "arXiv",
   eprint = {1801.02634},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, methods: statistical, reference systems },
     year = 2018,
    month = sep,
   volume = 156,
      eid = {123},
    pages = {123},
      doi = {10.3847/1538-3881/aabc4f},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..123A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{astropy2013,
   author = {{Astropy Collaboration} and {Robitaille}, T.~P. and {Tollerud}, E.~J. and
	{Greenfield}, P. and {Droettboom}, M. and {Bray}, E. and {Aldcroft}, T. and
	{Davis}, M. and {Ginsburg}, A. and {Price-Whelan}, A.~M. and
	{Kerzendorf}, W.~E. and {Conley}, A. and {Crighton}, N. and
	{Barbary}, K. and {Muna}, D. and {Ferguson}, H. and {Grollier}, F. and
	{Parikh}, M.~M. and {Nair}, P.~H. and {Unther}, H.~M. and {Deil}, C. and
	{Woillez}, J. and {Conseil}, S. and {Kramer}, R. and {Turner}, J.~E.~H. and
	{Singer}, L. and {Fox}, R. and {Weaver}, B.~A. and {Zabalza}, V. and
	{Edwards}, Z.~I. and {Azalee Bostroem}, K. and {Burke}, D.~J. and
	{Casey}, A.~R. and {Crawford}, S.~M. and {Dencheva}, N. and
	{Ely}, J. and {Jenness}, T. and {Labrie}, K. and {Lim}, P.~L. and
	{Pierfederici}, F. and {Pontzen}, A. and {Ptak}, A. and {Refsdal}, B. and
	{Servillat}, M. and {Streicher}, O.},
    title = "{Astropy: A community Python package for astronomy}",
  journal = {A\&A},
archivePrefix = "arXiv",
   eprint = {1307.6212},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A33},
    pages = {A33},
      doi = {10.1051/0004-6361/201322068},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2013A\%26A...558A..33A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/corner.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{corner,
       author = {{Foreman-Mackey}, Daniel},
        title = "{corner.py: Scatterplot matrices in Python}",
      journal = {JOSS},
         year = "2016",
        month = "Jun",
       volume = {1},
        pages = {24},
          doi = {10.21105/joss.00024},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016JOSS....1...24F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/cython.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{cython2011,
       author = {{Behnel}, Stefan and {Bradshaw}, Robert and {Citro}, Craig and {Dalcin}, Lisandro and {Seljebotn}, Dag Sverre and {Smith}, Kurt},
        title = "{Cython: The Best of Both Worlds}",
      journal = {Computing in Science and Engineering},
         year = 2011,
        month = mar,
       volume = {13},
       number = {2},
        pages = {31-39},
          doi = {10.1109/MCSE.2010.118},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011CSE....13b..31B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/fftw.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{fftw,
   author = {M. {Frigo} and S. G. {Johnson}},
  journal = {IEEE Proc.},
    title = {The Design and Implementation of FFTW3},
     year = {2005},
   volume = {93},
   number = {2},
    pages = {216-231},
      doi = {10.1109/JPROC.2004.840301},
     ISSN = {0018-9219},
    month = {Feb},
}


==> reproduce/software/bibtex/galsim.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{galsim,
       author = {{Rowe}, B.~T.~P. and {Jarvis}, M. and {Mandelbaum}, R. and
         {Bernstein}, G.~M. and {Bosch}, J. and {Simet}, M. and {Meyers}, J.~E. and
         {Kacprzak}, T. and {Nakajima}, R. and {Zuntz}, J. and {Miyatake}, H. and
         {Dietrich}, J.~P. and {Armstrong}, R. and {Melchior}, P. and
         {Gill}, M.~S.~S.},
        title = "{GALSIM: The modular galaxy image simulation toolkit}",
      journal = {Astron.Comput.},
     keywords = {Methods: data analysis, Techniques: image processing, Gravitational lensing, Cosmology: observations, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, 85-04},
         year = "2015",
        month = "Apr",
       volume = {10},
        pages = {121-150},
          doi = {10.1016/j.ascom.2015.02.002},
archivePrefix = {arXiv},
       eprint = {1407.7676},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&C....10..121R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/gnuastro.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{gnuastro,
       author = {{Akhlaghi}, Mohammad and {Ichikawa}, Takashi},
        title = "{Noise-based Detection and Segmentation of Nebulous Objects}",
      journal = {ApJS},
     keywords = {galaxies: irregular, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = sep,
       volume = {220},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.1088/0067-0049/220/1/1},
archivePrefix = {arXiv},
       eprint = {1505.01664},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..220....1A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/healpix.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{healpix,
       author = {{G{\'o}rski}, K.~M. and {Hivon}, E. and {Banday}, A.~J. and {Wandelt}, B.~D. and {Hansen}, F.~K. and {Reinecke}, M. and {Bartelmann}, M.},
        title = "{HEALPix: A Framework for High-Resolution Discretization and Fast Analysis of Data Distributed on the Sphere}",
      journal = {ApJ},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations, Methods: Statistical, Astrophysics},
         year = 2005,
        month = apr,
       volume = {622},
       number = {2},
        pages = {759-771},
          doi = {10.1086/427976},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409513},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...622..759G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/imfit.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{imfit2015,
       author = {{Erwin}, Peter},
        title = "{IMFIT: A Fast, Flexible New Program for Astronomical Image Fitting}",
      journal = {ApJ},
     keywords = {galaxies: bulges, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = feb,
       volume = {799},
       number = {2},
          eid = {226},
        pages = {226},
          doi = {10.1088/0004-637X/799/2/226},
archivePrefix = {arXiv},
       eprint = {1408.1097},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...799..226E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/kiwisolver.tex <==
%% Copyright (C) 2025-2025 Boud Roukema <boud@cosmo.torun.pl>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{cassowary2001,
   author = {{Grudin}, Jonathan and {Badros}, Greg J. and {Borning}, Alan and {Stuckey}, Peter J.},
    title = "{The Cassowary linear arithmetic constraint solving algorithm}",
    journal = {ACM Transactions on Computer-Human Interaction},
       year = 2001,
      month = dec,
     volume = {8},
     number = {4},
      pages = {267-306},
        doi = {10.1145/504704.504705},
}


==> reproduce/software/bibtex/matplotlib.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{matplotlib2007,
       author = {{Hunter}, John D.},
        title = "{Matplotlib: A 2D Graphics Environment}",
      journal = {CiSE},
     keywords = {Python, Scripting languages, Application development, Scientific programming},
         year = 2007,
        month = may,
       volume = {9},
       number = {3},
        pages = {90-95},
          doi = {10.1109/MCSE.2007.55},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007CSE.....9...90H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/missfits.tex <==
%% Copyright (C) 2020-2025 Surena Fatemi <surena.fatemi@ipm.ir>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{missfits,
       author = {{Marmo}, C. and {Bertin}, E.},
        title = "{MissFITS and WeightWatcher: Two Optimised Tools for Managing FITS Data.}",
      journal = {ASPC},
         year = 2008,
       volume = {394},
       series = {Astronomical Society of the Pacific Conference Series},
        pages = {619},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ASPC..394..619M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/mpi4py.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{mpi4py2011,
       author = {{Dalcin}, Lisandro D. and {Paz}, Rodrigo R. and {Kler}, Pablo A. and {Cosimo}, Alejandro},
        title = "{Parallel distributed computing using Python}",
      journal = {Advances in Water Resources},
         year = 2011,
        month = sep,
       volume = {34},
       number = {9},
        pages = {1124-1139},
          doi = {10.1016/j.advwatres.2011.04.013},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011AdWR...34.1124D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/numpy.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{numpy2020,
       author = {{Harris}, Charles R. and {Millman}, K. Jarrod and {van der Walt}, St{\'e}fan J. and {Gommers}, Ralf and {Virtanen}, Pauli and {Cournapeau}, David and {Wieser}, Eric and {Taylor}, Julian and {Berg}, Sebastian and {Smith}, Nathaniel J. and {Kern}, Robert and {Picus}, Matti and {Hoyer}, Stephan and {van Kerkwijk}, Marten H. and {Brett}, Matthew and {Haldane}, Allan and {del R{\'\i}o}, Jaime Fern{\'a}ndez and {Wiebe}, Mark and {Peterson}, Pearu and {G{\'e}rard-Marchant}, Pierre and {Sheppard}, Kevin and {Reddy}, Tyler and {Weckesser}, Warren and {Abbasi}, Hameer and {Gohlke}, Christoph and {Oliphant}, Travis E.},
        title = "{Array programming with NumPy}",
      journal = {Nature},
     keywords = {Computer Science - Mathematical Software, Statistics - Computation},
         year = 2020,
        month = sep,
       volume = {585},
       number = {7825},
        pages = {357-362},
          doi = {10.1038/s41586-020-2649-2},
archivePrefix = {arXiv},
       eprint = {2006.10256},
 primaryClass = {cs.MS},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020Natur.585..357H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/r-cran.tex <==
%% Copyright (C) 2022-2025 Boud Roukema <boud@cosmo.torun.pl>
%% Copyright (C) 2022-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{RIhakaGentleman1996,
      author = {{Ihaka}, Ross and {Gentleman}, Robert},
       title = "{R: A language for data analysis and graphics}",
     journal = {J.Comput.Graph.Stat.},
        year = {1996},
      volume = {5},
      number = {3},
       pages = {299-314},
         DOI = {10.1080/10618600.1996.10474713},
        ISSN = {10618600},
}


==> reproduce/software/bibtex/scamp.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{scamp,
   author = {{Bertin}, E.},
    title = "{Automatic Astrometric and Photometric Calibration with SCAMP}",
     year = 2006,
   journal= {ASPConf},
   volume = 351,
    month = jul,
    pages = {112},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2006ASPC..351..112B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/scipy.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{scipy2020,
       author = {{Virtanen}, Pauli and {Gommers}, Ralf and {Oliphant}, Travis E. and {Haberland}, Matt and {Reddy}, Tyler and {Cournapeau}, David and {Burovski}, Evgeni and {Peterson}, Pearu and {Weckesser}, Warren and {Bright}, Jonathan and {van der Walt}, St{\'e}fan J. and {Brett}, Matthew and {Wilson}, Joshua and {Millman}, K. Jarrod and {Mayorov}, Nikolay and {Nelson}, Andrew R.~J. and {Jones}, Eric and {Kern}, Robert and {Larson}, Eric and {Carey}, C.~J. and {Polat}, {\.I}lhan and {Feng}, Yu and {Moore}, Eric W. and {VanderPlas}, Jake and {Laxalde}, Denis and {Perktold}, Josef and {Cimrman}, Robert and {Henriksen}, Ian and {Quintero}, E.~A. and {Harris}, Charles R. and {Archibald}, Anne M. and {Ribeiro}, Ant{\^o}nio H. and {Pedregosa}, Fabian and {van Mulbregt}, Paul and {SciPy 1. 0 Contributors}},
        title = "{SciPy 1.0: fundamental algorithms for scientific computing in Python}",
      journal = {Nature Methods},
     keywords = {Computer Science - Mathematical Software, Computer Science - Data Structures and Algorithms, Computer Science - Software Engineering, Physics - Computational Physics},
         year = 2020,
        month = feb,
       volume = {17},
        pages = {261-272},
          doi = {10.1038/s41592-019-0686-2},
archivePrefix = {arXiv},
       eprint = {1907.10121},
 primaryClass = {cs.MS},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NatMe..17..261V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sextractor.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{sextractor,
       author = {{Bertin}, E. and {Arnouts}, S.},
        title = "{SExtractor: Software for source extraction.}",
      journal = {A\&AS},
     keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
         year = 1996,
        month = jun,
       volume = {117},
        pages = {393-404},
          doi = {10.1051/aas:1996164},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&AS..117..393B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sip_tpv.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{sip-tpv,
   author = {{Shupe}, D.~L. and {Laher}, R.~R. and {Storrie-Lombardi}, L. and
	{Surace}, J. and {Grillmair}, C. and {Levitan}, D. and {Sesar}, B.
	},
    title = "{More flexibility in representing geometric distortion in astronomical images}",
     year = 2012,
   journal = {SPIE},
   volume = 8451,
    month = sep,
      eid = {84511M},
    pages = {84511M},
      doi = {10.1117/12.925460},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2012SPIE.8451E..1MS},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/swarp.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{swarp,
   author = {{Bertin}, E. and {Mellier}, Y. and {Radovich}, M. and {Missonnier}, G. and
    {Didelon}, P. and {Morin}, B.},
  journal = {ASPConf},
    title = "{The TERAPIX Pipeline}",
     year = {2002},
   volume = {281},
    pages = {228},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2002ASPC..281..228B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sympy.tex <==
%% Copyright (C) 2019-2025 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@article{sympy,
 title = {SymPy: symbolic computing in Python},
 author = {Meurer, Aaron and Smith, Christopher P. and Paprocki, Mateusz and \v{C}ert\'{i}k, Ond\v{r}ej and Kirpichev, Sergey B. and Rocklin, Matthew and Kumar, AMiT and Ivanov, Sergiu and Moore, Jason K. and Singh, Sartaj and Rathnayake, Thilina and Vig, Sean and Granger, Brian E. and Muller, Richard P. and Bonazzi, Francesco and Gupta, Harsh and Vats, Shivam and Johansson, Fredrik and Pedregosa, Fabian and Curry, Matthew J. and Terrel, Andy R. and Rou\v{c}ka, \v{S}t\v{e}p\'{a}n and Saboo, Ashutosh and Fernando, Isuru and Kulal, Sumith and Cimrman, Robert and Scopatz, Anthony},
 year = 2017,
 month = jan,
 keywords = {Python, Computer algebra system, Symbolics},
 volume = 3,
 pages = {103},
 journal = {PeerJ CompSci},
 issn = {2376-5992},
 url = {https://doi.org/10.7717/peerj-cs.103},
 doi = {10.7717/peerj-cs.103}
}


==> reproduce/software/bibtex/tides.tex <==
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{tides,
   author = {{Abad}, A. and {Barrio}, R. and {Belsa}, F. and {Rodriguez}, M},
    title = "{Algorithm 924: TIDES, a Taylor Series Integrator for Differential EquationS}",
  journal = {ACM TOMS},
     year = 2012,
    month = nov,
   volume = 39,
      eid = {5},
    pages = {1-28},
      doi = {10.1145/2382585.2382590},
 keywords = {Taylor series method, automatic differentiation, high precision, numerical integration of ODEs, variational equations},
}


==> reproduce/software/shell/git-post-checkout <==
#!@BINDIR@/bash
#
# The example hook script to store the metadata information of version
# controlled files (with each commit) using the 'metastore' program.
#
# Copyright (C) 2016 Przemyslaw Pawelczyk <przemoc@gmail.com>
# Copyright (C) 2018-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# This script is taken from the 'examples/hooks/pre-commit' file of the
# 'metastore' package (installed within the project, with an MIT license
# for copyright). We have just changed the name of the 'MSFILE' and also
# set special characters for the installation location of meta-store so our
# own installation is found by Git.
#
# Permission is hereby granted, free of charge, to any person obtaining a
# copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to permit
# persons to whom the Software is furnished to do so, subject to the
# following conditions:
#
# The above copyright notice and this permission notice shall be included
# in all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS
# OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN
# NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
# DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR
# OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE
# USE OR OTHER DEALINGS IN THE SOFTWARE.


# File containig the metadata and metastore executable.
MSFILE=".file-metadata"
MSBIN=@BINDIR@/metastore

# If metastore is not installed, then ignore this script (exit with a
# status of 0).
if [ ! -f $MSBIN ]; then exit 0; fi

# Delete all temporary files
find @TOP_PROJECT_DIR@/ -name "*~" -type f -delete

# Function to help in reporting a crash.
exit_on_fail() {
	"$@"
	if [ $? -ne 0 ]; then
		echo "Failed to execute: $@" >&2
		exit 1
	fi
}

# Check if the metadata file exists.
if [ ! -e "$MSFILE" ]; then
	echo "\"$MSFILE\" missing" >&2
	exit 1
fi

# Run metastore.
exit_on_fail \
       $MSBIN -a -m -e -E -q -O @USER@ -G @GROUP@ -f "$MSFILE"

# Return with a success code (0).
exit 0


==> reproduce/software/shell/git-pre-commit <==
#!@BINDIR@/bash
#
# The example hook script to store the metadata information of version
# controlled files (with each commit) using the 'metastore' program.
#
# Copyright (C) 2016 Przemyslaw Pawelczyk <przemoc@gmail.com>
# Copyright (C) 2018-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# WARNING:
#
# If the commit is aborted (e.g. by not entering any synopsis),
# then updated metastore file (.metadata by default) is not reverted,
# so its new version remains in the index.
# To undo any changes in metastore file written since HEAD commit,
# you may want to reset and checkout HEAD version of the file:
#
#     git reset HEAD -- .metadata
#     git checkout HEAD -- .metadata
#
# This script is taken from the 'examples/hooks/pre-commit' file of the
# 'metastore' package (installed within the project, with an MIT license
# for copyright). Here, the name of the 'MSFILE' and also set special
# characters for the installation location of meta-store so our own
# installation is found by Git.
#
# Permission is hereby granted, free of charge, to any person obtaining a
# copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to permit
# persons to whom the Software is furnished to do so, subject to the
# following conditions:
#
# The above copyright notice and this permission notice shall be included
# in all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS
# OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN
# NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
# DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR
# OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE
# USE OR OTHER DEALINGS IN THE SOFTWARE.

# File containig the metadata and metastore executable.
MSFILE=".file-metadata"
MSBIN=@BINDIR@/metastore

# If metastore is not installed, then ignore this script (exit with a
# status of 0).
if [ ! -f $MSBIN ]; then exit 0; fi

# Function to help in reporting a crash.
exit_on_fail() {
	"$@"
	if [ $? -ne 0 ]; then
		echo "Failed to execute: $@" >&2
		exit 1
	fi
}

# Run metastore.
exit_on_fail \
	$MSBIN -O @USER@ -G @GROUP@ -s -f "$MSFILE"

# If it's first metastore commit, store again to include $MSFILE in $MSFILE.
if ! git-ls-tree --name-only HEAD 2>/dev/null | grep -Fqx "$MSFILE"; then
	exit_on_fail \
	        $MSBIN -O @USER@ -G @GROUP@ -s -f "$MSFILE"
fi

# Check if the metadata file exists.
if [ ! -e "$MSFILE" ]; then
	echo "\"$MSFILE\" missing" >&2
	exit 1
fi

# Add the metadata file to the Git repository.
exit_on_fail \
	git-add "$MSFILE"

# Return with a success code (0).
exit 0


==> tex/build/macros/dependencies-bib.tex <==


@ARTICLE{gnuastro,
       author = {{Akhlaghi}, Mohammad and {Ichikawa}, Takashi},
        title = "{Noise-based Detection and Segmentation of Nebulous Objects}",
      journal = {ApJS},
     keywords = {galaxies: irregular, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = sep,
       volume = {220},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.1088/0067-0049/220/1/1},
archivePrefix = {arXiv},
       eprint = {1505.01664},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..220....1A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> tex/src/preamble-biblatex.tex <==
%% Biblatex settings.
%%
%% Settings necessary to make the bibliography with Biblatex. Keeping all
%% BibLaTeX settings in a separate preamble was done in the spirit of
%% modularity to 1) easily managable, 2) If a similar BibLaTeX
%% configuration is necessary in another LaTeX compilation, this file can
%% just be copied there and used.
%%
%% USAGE:
%%  - 'tex/src/references.tex': the file containing Bibtex source of each
%%     reference. The file suffix doesn't have to be '.bib'. This naming
%%     helps in clearly identifying the files and avoiding places that
%%     complain about '.bib' files.
%
%% Copyright (C) 2018-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%
%% This file is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the
%% Free Software Foundation, either version 3 of the License, or (at your
%% option) any later version.
%
%% This file is distributed in the hope that it will be useful, but WITHOUT
%% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General Public License
%% for more details.
%
%% You should have received a copy of the GNU General Public License along
%% with this file.  If not, see <http://www.gnu.org/licenses/>.




%% To break up highlighted text (for example texttt when some it is on the
%% line break) and also to no underline emphasized words (like journal
%% titles in the references).
\usepackage[normalem]{ulem}





%% For quotation signs (sometimes used by BibLaTeX)
\usepackage{csquotes}





%% To define colors
\usepackage{xcolor}





% Basic BibLaTeX settings
\usepackage[
    doi=false,
    url=false,
    dashed=false,
    eprint=false,
    maxbibnames=2,
    minbibnames=1,
    hyperref=true,
    maxcitenames=2,
    mincitenames=1,
    giveninits=true,
    style=authoryear,
    uniquelist=false,
    backend=biber,natbib]{biblatex}
\DeclareFieldFormat[article]{pages}{#1}
\DeclareFieldFormat{pages}{\mkfirstpage[{\mkpageprefix[bookpagination]}]{#1}}
\addbibresource{tex/src/references.tex}
\addbibresource{tex/build/macros/dependencies-bib.tex}
\renewbibmacro{in:}{}
\AtEveryBibitem{\clearfield{month}}
\renewcommand*{\bibfont}{\footnotesize}
\DefineBibliographyStrings{english}{references = {References}}

%% Include the adsurl field key into those that are recognized:
\DeclareSourcemap{
  \maps[datatype=bibtex]{
    \map{
      \step[fieldsource=adsurl,fieldtarget=iswc]
      \step[fieldsource=gbkurl,fieldtarget=iswc]
    }
  }
}

%% Set the color of the doi link to mymg (magenta) and the ads links
%% to mypurp (or purple):
\definecolor{mypurp}{cmyk}{0.75,1,0,0}
\newcommand{\doihref}[2]{\href{#1}{\color{magenta}{#2}}}
\newcommand{\adshref}[2]{\href{#1}{\color{mypurp}{#2}}}
\newcommand{\blackhref}[2]{\href{#1}{\color{black}{#2}}}

%% Define a format for the printtext commands in
%% DeclareBibliographyDriver to make links for the doi, ads link and
%% arxiv link:
\DeclareFieldFormat{doilink}{
  \iffieldundef{doi}{#1}{\doihref{http://dx.doi.org/\thefield{doi}}{#1}}}
\DeclareFieldFormat{adslink}{
    \iffieldundef{iswc}{#1}{\adshref{\thefield{iswc}}{#1}}}
\DeclareFieldFormat{arxivlink}{
  \iffieldundef{eprint}{#1}{\href{http://arxiv.org/abs/\thefield{eprint}}{#1}}}

\DeclareListFormat{doiforbook}{
  \iffieldundef{doi}{#1}{\doihref{http://dx.doi.org/\thefield{doi}}{#1}}}
\DeclareFieldFormat{googlebookslink}{
    \iffieldundef{iswc}{#1}{\adshref{\thefield{iswc}}{#1}}}

%% Set the formatting to make the last three values into the
%% appropriate link. Note that the % signs are necessary. Without
%% them, the items will be indented.
\DeclareBibliographyDriver{article}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \usebibmacro{author/translator+others}%
  \newunit%
  \ifdefined\makethesis\printtext{\usebibmacro{title}}\fi%
  \newunit%
  \printtext[doilink]{\usebibmacro{journal}}%
  \addcomma%
  \printtext[adslink]{\printfield{volume}}%
  \addcomma%
  \printtext[arxivlink]{\printfield{pages}}%
  \addperiod%
}

\DeclareBibliographyDriver{book}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \usebibmacro{author/translator+others}%
  \newunit%
  \printtext{\usebibmacro{title}}%
  \addperiod%
  \addspace%
  \printlist[doiforbook]{publisher}%
  \addcomma%
  \addspace%
  \printfield[googlebookslink]{edition}%
  \printtext{ ed.}%
  \addperiod%
}

%% In order to have et al. instead of et al.,:
\renewcommand*{\nameyeardelim}{\addspace}


==> tex/src/preamble-maneage-default-style.tex <==
%% General paper's style settings.
%
%% This preamble can be completely ignored when including this TeX file in
%% another style. This is done because this LaTeX build is meant to be an
%% initial/internal phase or part of a larger effort, so it has a basic
%% style defined here as a preamble. To ignore it, uncomment or delete the
%% respective line in 'paper.tex'.
%
%% Copyright (C) 2019-2025 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%
%% This file is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the
%% Free Software Foundation, either version 3 of the License, or (at your
%% option) any later version.
%
%% This file is distributed in the hope that it will be useful, but WITHOUT
%% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General Public License
%% for more details.
%
%% You should have received a copy of the GNU General Public License along
%% with this file.  If not, see <http://www.gnu.org/licenses/>.





%% Font.
\usepackage[T1]{fontenc}
\usepackage{newtxtext}
\usepackage{newtxmath}





%% Print size
\usepackage[a4paper, includeheadfoot, body={18.7cm, 24.5cm}]{geometry}





%% Set the distance between the columns if two columns:
\setlength{\columnsep}{0.75cm}





% To allow figures to take up more space on the top of the page:
\renewcommand{\topfraction}{.99}
\renewcommand{\bottomfraction}{.7}
\renewcommand{\textfraction}{.05}
\renewcommand{\floatpagefraction}{.99}
\renewcommand{\dbltopfraction}{.99}
\renewcommand{\dblfloatpagefraction}{.99}
\setcounter{topnumber}{1}
\setcounter{bottomnumber}{0}
\setcounter{totalnumber}{2}
\setcounter{dbltopnumber}{1}





%% To make the footnotes align:
\usepackage[hang]{footmisc}
\setlength\footnotemargin{10pt}





%For including time in the title:
\usepackage{datetime}





%% Define the abstract environment
\renewenvironment{abstract}
 {\vspace{-0.5cm}\small%
  \list{}{%
    \setlength{\leftmargin}{2cm}%
    \setlength{\rightmargin}{\leftmargin}%
  }%
  \item\relax}
 {\endlist}





%% To keep the main page's code clean.
\newcommand{\includeabstract}[1]{%
\twocolumn[%
  \begin{@twocolumnfalse}%
    \maketitle%
    \begin{abstract}%
    #1%
    \end{abstract}%
    \vspace{1cm}%
  \end{@twocolumnfalse}%
  ]%
}





%% Basic header style
%% ------------------
%
%% The steps below are to use the necessary LaTeX packages to get the demo
%% Maneage paper running with a reasonably looking, custom paper style. If
%% you are using a custom journal style, feel free to delete these.

%% General page header settings.
\usepackage{fancyhdr}
\pagestyle{fancy}
\lhead{\footnotesize{\scshape Draft paper}, {\footnotesize nnn:i (pp), Year Month day}}
\rhead{\scshape\footnotesize YOUR-NAME et al.}
\cfoot{\thepage}
\setlength{\voffset}{0.75cm}
\setlength{\headsep}{0.2cm}
\setlength{\footskip}{0.75cm}
\renewcommand{\headrulewidth}{0pt}

%% Specific style for first page.
\fancypagestyle{firststyle}
{
  \lhead{\footnotesize{\scshape Draft paper}, nnn:i (pp), YYYY Month day\\
  \scriptsize \textcopyright YYYY, Your name. All rights reserved.}
  \rhead{\footnotesize \footnotesize \today, \currenttime\\}
}

%To set the style of the titles:
\usepackage{titlesec}
\titleformat{\section}
  {\centering\normalfont\uppercase}
  {\thesection.}
  {0em}
  { }
\titleformat{\subsection}
  {\centering\normalsize\slshape}
  {\thesubsection.}
  {0em}
  { }
\titleformat{\subsubsection}
  {\centering\small\slshape}
  {\thesubsubsection.}
  {0em}
  { }

%% Title and author information
\usepackage{authblk}
\renewcommand\Authfont{\small\scshape}
\renewcommand\Affilfont{\footnotesize\normalfont}
\setlength{\affilsep}{0.2cm}


==> tex/src/references.tex <==
%% Non-software BibTeX entries. The software-specific BibTeX entries are
%% stored in a '*.tex' file under the 'tex/dependencies' directory.
%
%% [[[BibTeX 0.99d complains with the at-character, even when its in a
%%    comment line! So ::at:: is used instead in the email address]]].
%% Copyright (C) 2024-2025 Mohammad Akhlaghi <mohammad::at::akhlaghi.org>
%% Copyright (C) 2024-2025 Sepideh Eskandarlou <sepideh.eskandarlou::at::gmail.com>
%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.




@ARTICLE{huillier12,
       author = {{{L\textquoteright}Huillie}, B. and {Combes}, F. and {Semelin}, B.},
        title = "{Mass assembly of galaxies: Smooth accretion versus mergers}",
      journal = {A\&A},
     keywords = {galaxies: formation, galaxies: evolution, galaxies: interactions, galaxies: halos, galaxies: star formation, galaxies: structure, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2012,
        month = aug,
       volume = {544},
          eid = {A68},
        pages = {A68},
          doi = {10.1051/0004-6361/201117924},
archivePrefix = {arXiv},
       eprint = {1108.4247},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A\&A...544A..68L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{maneage,
       author = {{Akhlaghi}, Mohammad and {Infante-Sainz}, Raul and
         {Roukema}, Boudewijn F. and {Khellat}, Mohammadreza and
         {Valls-Gabaud}, David and {Baena-Galle}, Roberto},
        title = "{Toward Long-Term and Archivable Reproducibility}",
      journal = {CiSE},
     keywords = {Computer Science - Digital Libraries},
         year = 2021,
        month = may,
       volume = {23},
       number = {3},
        pages = {82-91},
          doi = {10.1109/MCSE.2021.3072860},
archivePrefix = {arXiv},
       eprint = {2006.03018},
 primaryClass = {cs.DL},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021CSE....23c..82A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{phangsmuse,
       author = {{Emsellem}, Eric and {Schinnerer}, Eva and {Santoro}, Francesco and {Belfiore}, Francesco and {Pessa}, Ismael and {McElroy}, Rebecca and {Blanc}, Guillermo A. and {Congiu}, Enrico and {Groves}, Brent and {Ho}, I. -Ting and {Kreckel}, Kathryn and {Razza}, Alessandro and {Sanchez-Blazquez}, Patricia and {Egorov}, Oleg and {Faesi}, Chris and {Klessen}, Ralf S. and {Leroy}, Adam K. and {Meidt}, Sharon and {Querejeta}, Miguel and {Rosolowsky}, Erik and {Scheuermann}, Fabian and {Anand}, Gagandeep S. and {Barnes}, Ashley T. and {Be{\v{s}}li{\'c}}, Ivana and {Bigiel}, Frank and {Boquien}, M{\'e}d{\'e}ric and {Cao}, Yixian and {Chevance}, M{\'e}lanie and {Dale}, Daniel A. and {Eibensteiner}, Cosima and {Glover}, Simon C.~O. and {Grasha}, Kathryn and {Henshaw}, Jonathan D. and {Hughes}, Annie and {Koch}, Eric W. and {Kruijssen}, J.~M. Diederik and {Lee}, Janice and {Liu}, Daizhong and {Pan}, Hsi-An and {Pety}, J{\'e}r{\^o}me and {Saito}, Toshiki and {Sandstrom}, Karin M. and {Schruba}, Andreas and {Sun}, Jiayi and {Thilker}, David A. and {Usero}, Antonio and {Watkins}, Elizabeth J. and {Williams}, Thomas G.},
        title = "{The PHANGS-MUSE survey. Probing the chemo-dynamical evolution of disc galaxies}",
      journal = {A\&A},
     keywords = {galaxies: spiral, galaxies: star formation, surveys, techniques: imaging spectroscopy, ISM: general, stars: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2022,
        month = mar,
       volume = {659},
          eid = {A191},
        pages = {A191},
          doi = {10.1051/0004-6361/202141727},
archivePrefix = {arXiv},
       eprint = {2110.03708},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...659A.191E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{planckcollab18,
       author = {{Planck Collaboration} and {Aghanim}, N. and {Akrami}, Y. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basak}, S. and {Battye}, R. and {Benabed}, K. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Carron}, J. and {Challinor}, A. and {Chiang}, H.~C. and {Chluba}, J. and {Colombo}, L.~P.~L. and {Combet}, C. and {Contreras}, D. and {Crill}, B.~P. and {Cuttaia}, F. and {de Bernardis}, P. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {Di Valentino}, E. and {Diego}, J.~M. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Dusini}, S. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Fantaye}, Y. and {Farhang}, M. and {Fergusson}, J. and {Fernandez-Cobos}, R. and {Finelli}, F. and {Forastieri}, F. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and {Ghosh}, T. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hamann}, J. and {Handley}, W. and {Hansen}, F.~K. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Huang}, Z. and {Jaffe}, A.~H. and {Jones}, W.~C. and {Karakci}, A. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kiiveri}, K. and {Kim}, J. and {Kisner}, T.~S. and {Knox}, L. and {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Lemos}, P. and {Lesgourgues}, J. and {Levrier}, F. and {Lewis}, A. and {Liguori}, M. and {Lilje}, P.~B. and {Lilley}, M. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marcos-Caballero}, A. and {Maris}, M. and {Martin}, P.~G. and {Martinelli}, M. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {Mauri}, N. and {McEwen}, J.~D. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Mennella}, A. and {Migliaccio}, M. and {Millea}, M. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Montier}, L. and {Morgante}, G. and {Moss}, A. and {Natoli}, P. and {N{\o}rgaard-Nielsen}, H.~U. and {Pagano}, L. and {Paoletti}, D. and {Partridge}, B. and {Patanchon}, G. and {Peiris}, H.~V. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Polastri}, L. and {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Salvati}, L. and {Sandri}, M. and {Savelainen}, M. and {Scott}, D. and {Shellard}, E.~P.~S. and {Sirignano}, C. and {Sirri}, G. and {Spencer}, L.~D. and {Sunyaev}, R. and {Suur-Uski}, A. -S. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Tenti}, M. and {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vibert}, L. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {White}, M. and {White}, S.~D.~M. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2018 results. VI. Cosmological parameters}",
      journal = {A\&A},
     keywords = {cosmic background radiation, cosmological parameters, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A6},
        pages = {A6},
          doi = {10.1051/0004-6361/201833910},
archivePrefix = {arXiv},
       eprint = {1807.06209},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A...6P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{alliez19,
       author = {{Alliez}, Pierre and {Di Cosmo}, Roberto and {Guedj}, Benjamin and
         {Girault}, Alain and {Hacid}, Mohand-Said and {Legrand}, Arnaud and
         {Rougier}, Nicolas P.},
        title = "{Attributing and Referencing (Research) Software: Best Practices and Outlook from Inria}",
      journal = {CiSE},
       volume = {22},
         year = "2020",
        month = "Jan",
        pages = {39-52},
archivePrefix = {arXiv},
       eprint = {1905.11123},
 primaryClass = {cs.DL},
          doi = {10.1109/MCSE.2019.2949413},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190511123A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{infantesainz20,
       author = {{Infante-Sainz}, Ra{\'u}l and {Trujillo}, Ignacio and
         {Rom{\'a}n}, Javier},
        title = "{The Sloan Digital Sky Survey extended point spread functions}",
      journal = {MNRAS},
         year = 2020,
        month = feb,
       volume = {491},
       number = {4},
        pages = {5317-5329},
          doi = {10.1093/mnras/stz3111},
archivePrefix = {arXiv},
       eprint = {1911.01430},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.491.5317I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{akhlaghi19,
       author = {{Akhlaghi}, Mohammad},
        title = "{Carving out the low surface brightness universe with NoiseChisel}",
      journal = {IAU Symposium 335},
         year = 2019,
        month = sep,
          eid = {arXiv:1909.11230},
        pages = {arXiv:1909.11230},
archivePrefix = {arXiv},
       eprint = {1909.11230},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190911230A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{dey19,
       author = {{Dey}, Arjun and {Schlegel}, David J. and {Lang}, Dustin and {Blum}, Robert and {Burleigh}, Kaylan and {Fan}, Xiaohui and {Findlay}, Joseph R. and {Finkbeiner}, Doug and {Herrera}, David and {Juneau}, St{\'e}phanie and {Landriau}, Martin and {Levi}, Michael and {McGreer}, Ian and {Meisner}, Aaron and {Myers}, Adam D. and {Moustakas}, John and {Nugent}, Peter and {Patej}, Anna and {Schlafly}, Edward F. and {Walker}, Alistair R. and {Valdes}, Francisco and {Weaver}, Benjamin A. and {Y{\`e}che}, Christophe and {Zou}, Hu and {Zhou}, Xu and {Abareshi}, Behzad and {Abbott}, T.~M.~C. and {Abolfathi}, Bela and {Aguilera}, C. and {Alam}, Shadab and {Allen}, Lori and {Alvarez}, A. and {Annis}, James and {Ansarinejad}, Behzad and {Aubert}, Marie and {Beechert}, Jacqueline and {Bell}, Eric F. and {BenZvi}, Segev Y. and {Beutler}, Florian and {Bielby}, Richard M. and {Bolton}, Adam S. and {Brice{\~n}o}, C{\'e}sar and {Buckley-Geer}, Elizabeth J. and {Butler}, Karen and {Calamida}, Annalisa and {Carlberg}, Raymond G. and {Carter}, Paul and {Casas}, Ricard and {Castander}, Francisco J. and {Choi}, Yumi and {Comparat}, Johan and {Cukanovaite}, Elena and {Delubac}, Timoth{\'e}e and {DeVries}, Kaitlin and {Dey}, Sharmila and {Dhungana}, Govinda and {Dickinson}, Mark and {Ding}, Zhejie and {Donaldson}, John B. and {Duan}, Yutong and {Duckworth}, Christopher J. and {Eftekharzadeh}, Sarah and {Eisenstein}, Daniel J. and {Etourneau}, Thomas and {Fagrelius}, Parker A. and {Farihi}, Jay and {Fitzpatrick}, Mike and {Font-Ribera}, Andreu and {Fulmer}, Leah and {G{\"a}nsicke}, Boris T. and {Gaztanaga}, Enrique and {George}, Koshy and {Gerdes}, David W. and {Gontcho}, Satya Gontcho A. and {Gorgoni}, Claudio and {Green}, Gregory and {Guy}, Julien and {Harmer}, Diane and {Hernandez}, M. and {Honscheid}, Klaus and {Huang}, Lijuan Wendy and {James}, David J. and {Jannuzi}, Buell T. and {Jiang}, Linhua and {Joyce}, Richard and {Karcher}, Armin and {Karkar}, Sonia and {Kehoe}, Robert and {Kneib}, Jean-Paul and {Kueter-Young}, Andrea and {Lan}, Ting-Wen and {Lauer}, Tod R. and {Le Guillou}, Laurent and {Le Van Suu}, Auguste and {Lee}, Jae Hyeon and {Lesser}, Michael and {Perreault Levasseur}, Laurence and {Li}, Ting S. and {Mann}, Justin L. and {Marshall}, Robert and {Mart{\'\i}nez-V{\'a}zquez}, C.~E. and {Martini}, Paul and {du Mas des Bourboux}, H{\'e}lion and {McManus}, Sean and {Meier}, Tobias Gabriel and {M{\'e}nard}, Brice and {Metcalfe}, Nigel and {Mu{\~n}oz-Guti{\'e}rrez}, Andrea and {Najita}, Joan and {Napier}, Kevin and {Narayan}, Gautham and {Newman}, Jeffrey A. and {Nie}, Jundan and {Nord}, Brian and {Norman}, Dara J. and {Olsen}, Knut A.~G. and {Paat}, Anthony and {Palanque-Delabrouille}, Nathalie and {Peng}, Xiyan and {Poppett}, Claire L. and {Poremba}, Megan R. and {Prakash}, Abhishek and {Rabinowitz}, David and {Raichoor}, Anand and {Rezaie}, Mehdi and {Robertson}, A.~N. and {Roe}, Natalie A. and {Ross}, Ashley J. and {Ross}, Nicholas P. and {Rudnick}, Gregory and {Safonova}, Sasha and {Saha}, Abhijit and {S{\'a}nchez}, F. Javier and {Savary}, Elodie and {Schweiker}, Heidi and {Scott}, Adam and {Seo}, Hee-Jong and {Shan}, Huanyuan and {Silva}, David R. and {Slepian}, Zachary and {Soto}, Christian and {Sprayberry}, David and {Staten}, Ryan and {Stillman}, Coley M. and {Stupak}, Robert J. and {Summers}, David L. and {Sien Tie}, Suk and {Tirado}, H. and {Vargas-Maga{\~n}a}, Mariana and {Vivas}, A. Katherina and {Wechsler}, Risa H. and {Williams}, Doug and {Yang}, Jinyi and {Yang}, Qian and {Yapici}, Tolga and {Zaritsky}, Dennis and {Zenteno}, A. and {Zhang}, Kai and {Zhang}, Tianmeng and {Zhou}, Rongpu and {Zhou}, Zhimin},
        title = "{Overview of the DESI Legacy Imaging Surveys}",
      journal = {AJ},
     keywords = {catalogs, surveys, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = may,
       volume = {157},
       number = {5},
          eid = {168},
        pages = {168},
          doi = {10.3847/1538-3881/ab089d},
archivePrefix = {arXiv},
       eprint = {1804.08657},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....157..168D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@ARTICLE{martineza23,
       author = {{Mart{\'\i}nez-Delgado}, David and {Cooper}, Andrew P. and {Rom{\'a}n}, Javier and {Pillepich}, Annalisa and {Erkal}, Denis and {Pearson}, Sarah and {Moustakas}, John and {Laporte}, Chervin F.~P. and {Laine}, Seppo and {Akhlaghi}, Mohammad and {Lang}, Dustin and {Makarov}, Dmitry and {Borlaff}, Alejandro S. and {Donatiello}, Giuseppe and {Pearson}, William J. and {Mir{\'o}-Carretero}, Juan and {Cuillandre}, Jean-Charles and {Dom{\'\i}nguez}, Helena and {Roca-F{\`a}brega}, Santi and {Frenk}, Carlos S. and {Schmidt}, Judy and {G{\'o}mez-Flechoso}, Mar{\'\i}a A. and {Guzman}, Rafael and {Libeskind}, Noam I. and {Dey}, Arjun and {Weaver}, Benjamin A. and {Schlegel}, David and {Myers}, Adam D. and {Valdes}, Frank G.},
        title = "{Hidden depths in the local Universe: The Stellar Stream Legacy Survey}",
      journal = {A\&A},
     keywords = {galaxies: interactions, galaxies: dwarf, galaxies: formation, surveys, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = mar,
       volume = {671},
          eid = {A141},
        pages = {A141},
          doi = {10.1051/0004-6361/202245011},
archivePrefix = {arXiv},
       eprint = {2104.06071},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...671A.141M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{martinezb23,
       author = {{Mart{\'\i}nez-Delgado}, David and {Roca-F{\`a}brega}, Santi and {Mir{\'o}-Carretero}, Juan and {G{\'o}mez-Flechoso}, Maria Angeles and {Rom{\`a}n}, Javier and {Donatiello}, Giuseppe and {Schmidt}, Judy and {Lang}, Dustin and {Akhlaghi}, Mohammad and {Hanson}, Mark},
        title = "{A giant umbrella-like stellar stream around the tidal ring galaxy NGC 922}",
      journal = {A\&A},
     keywords = {galaxies: interactions, galaxies: structure, galaxies: clusters: individual: NGC 922, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = jan,
       volume = {669},
          eid = {A103},
        pages = {A103},
          doi = {10.1051/0004-6361/202244832},
archivePrefix = {arXiv},
       eprint = {2209.01583},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...669A.103M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{martinez10,
       author = {{Mart{\'\i}nez-Delgado}, David and {Gabany}, R. Jay and {Crawford}, Ken and {Zibetti}, Stefano and {Majewski}, Steven R. and {Rix}, Hans-Walter and {Fliri}, J{\"u}rgen and {Carballo-Bello}, Julio A. and {Bardalez-Gagliuffi}, Daniella C. and {Pe{\~n}arrubia}, Jorge and {Chonis}, Taylor S. and {Madore}, Barry and {Trujillo}, Ignacio and {Schirmer}, Mischa and {McDavid}, David A.},
        title = "{Stellar Tidal Streams in Spiral Galaxies of the Local Volume: A Pilot Survey with Modest Aperture Telescopes}",
      journal = {AJ},
     keywords = {dark matter, galaxies: dwarf, galaxies: evolution, galaxies: halos, galaxies: interactions, galaxies: structure, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2010,
        month = oct,
       volume = {140},
       number = {4},
        pages = {962-967},
          doi = {10.1088/0004-6256/140/4/962},
archivePrefix = {arXiv},
       eprint = {1003.4860},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010AJ....140..962M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{hood18,
       author = {{Hood}, Callie E. and {Kannappan}, Sheila J. and {Stark}, David V. and {Dell'Antonio}, Ian P. and {Moffett}, Amanda J. and {Eckert}, Kathleen D. and {Norris}, Mark A. and {Hendel}, David},
        title = "{The Origin of Faint Tidal Features around Galaxies in the RESOLVE Survey}",
      journal = {APJ},
     keywords = {galaxies: evolution, galaxies: interactions, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = apr,
       volume = {857},
       number = {2},
          eid = {144},
        pages = {144},
          doi = {10.3847/1538-4357/aab719},
archivePrefix = {arXiv},
       eprint = {1803.05447},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...857..144H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}









@ARTICLE{miro24b,
       author = {{Mir{\'o}-Carretero}, Juan and {G{\'o}mez-Flechoso}, Mar{\'\i}a A. and {Mart{\'\i}nez-Delgado}, David and {Cooper}, Andrew P. and {Roca-F{\`a}brega}, Santi and {Akhlaghi}, Mohammad and {Pillepich}, Annalisa and {Kuijken}, Konrad and {Erkal}, Denis and {Buck}, Tobias and {Hellwing}, Wojciech A. and {Bose}, Sownak and {Donatiello}, Giuseppe and {Frenk}, Carlos S.},
        title = "{Extragalactic stellar tidal streams: Observations meet simulation}",
      journal = {\aap},
     keywords = {galaxies: evolution, galaxies: halos, galaxies: photometry, cosmology: observations, dark matter, Astrophysics of Galaxies},
         year = 2025,
        month = aug,
       volume = {700},
          eid = {A176},
        pages = {A176},
          doi = {10.1051/0004-6361/202452791},
archivePrefix = {arXiv},
       eprint = {2409.03585},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2025A&A...700A.176M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}











@ARTICLE{miro24a,
       author = {{Mir{\'o}-Carretero}, Juan and {Mart{\'\i}nez-Delgado}, David and {G{\'o}mez-Flechoso}, Mar{\'\i}a A. and {Cooper}, Andrew and {Akhlaghi}, Mohammad and {Donatiello}, Giuseppe and {Kuijken}, Konrad and {Lang}, Dustin and {Makarov}, Dmitry and {Laine}, Seppo and {Roca-F{\`a}brega}, Santi},
        title = "{Extragalactic stellar tidal streams in the Dark Energy Survey}",
      journal = {\aap},
     keywords = {catalogs, galaxies: dwarf, galaxies: evolution, galaxies: interactions, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = nov,
       volume = {691},
          eid = {A196},
        pages = {A196},
          doi = {10.1051/0004-6361/202451685},
archivePrefix = {arXiv},
       eprint = {2407.20483},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A&A...691A.196M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{miro23,
       author = {{Mir{\'o}-Carretero}, Juan and {Mart{\'\i}nez-Delgado}, David and {Farr{\`a}s-Aloy}, S{\'\i}lvia and {G{\'o}mez-Flechoso}, Maria A. and {Cooper}, Andrew and {Roca-F{\`a}brega}, Santi and {Kuijken}, Konrad and {Akhlaghi}, Mohammad and {Donatiello}, Giuseppe},
        title = "{A search for stellar tidal streams around Milky Way analogues from the SAGA sample}",
      journal = {AAP},
     keywords = {galaxies: interactions, galaxies: dwarf, Galaxy: evolution, galaxies: photometry, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = jan,
       volume = {669},
          eid = {L13},
        pages = {L13},
          doi = {10.1051/0004-6361/202245003},
archivePrefix = {arXiv},
       eprint = {2209.08636},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...669L..13M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{bullock05,
       author = {{Bullock}, James S. and {Johnston}, Kathryn V.},
        title = "{Tracing Galaxy Formation with Stellar Halos. I. Methods}",
      journal = {APJ},
     keywords = {Cosmology: Dark Matter, Galaxies: Dwarf, Galaxies: Evolution, Galaxies: Formation, Galaxies: Halos, Galaxies: Kinematics and Dynamics, Galaxy: Evolution, Galaxy: Formation, Galaxy: Halo, Galaxy: Kinematics and Dynamics, Galaxies: Local Group, Astrophysics},
         year = 2005,
        month = dec,
       volume = {635},
       number = {2},
        pages = {931-949},
          doi = {10.1086/497422},
archivePrefix = {arXiv},
       eprint = {astro-ph/0506467},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...635..931B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{kauffmann93,
       author = {{Kauffmann}, G. and {White}, S.~D.~M. and {Guiderdoni}, B.},
        title = "{The formation and evolution of galaxies within merging dark matter haloes.}",
      journal = {MNRAS},
         year = 1993,
        month = sep,
       volume = {264},
        pages = {201-218},
          doi = {10.1093/mnras/264.1.201},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993MNRAS.264..201K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Cole00,
       author = {{Cole}, Shaun and {Lacey}, Cedric G. and {Baugh}, Carlton M. and {Frenk}, Carlos S.},
        title = "{Hierarchical galaxy formation}",
      journal = {MNRAS},
     keywords = {GALAXIES: FORMATION, Astrophysics},
         year = 2000,
        month = nov,
       volume = {319},
       number = {1},
        pages = {168-204},
          doi = {10.1046/j.1365-8711.2000.03879.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0007281},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000MNRAS.319..168C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{stringer07,
       author = {{Stringer}, M.~J. and {Benson}, A.~J.},
        title = "{The formation of galaxy discs in a hierarchical universe}",
      journal = {MNRAS},
     keywords = {stars: formation, galaxies: evolution, galaxies: formation, galaxies: halo, galaxies: kinematics and dynamics, galaxies: structure, Astrophysics},
         year = 2007,
        month = dec,
       volume = {382},
       number = {2},
        pages = {641-651},
          doi = {10.1111/j.1365-2966.2007.12469.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0703380},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.382..641S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{halton66,
       author = {{Arp}, Halton},
        title = "{Atlas of Peculiar Galaxies}",
      journal = {APJS},
         year = 1966,
        month = nov,
       volume = {14},
        pages = {1},
          doi = {10.1086/190147},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1966ApJS...14....1A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{toomre72,
       author = {{Toomre}, Alar and {Toomre}, Juri},
        title = "{Galactic Bridges and Tails}",
      journal = {APJ},
         year = 1972,
        month = dec,
       volume = {178},
        pages = {623-666},
          doi = {10.1086/151823},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1972ApJ...178..623T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{quinn84,
       author = {{Quinn}, P.~J.},
        title = "{On the formation and dynamics of shells around elliptical galaxies.}",
      journal = {APJ},
     keywords = {Elliptical Galaxies, Galactic Evolution, Galactic Structure, Halos, Astronomical Models, Disk Galaxies, Gravitational Effects, Many Body Problem, Time Response, Astrophysics},
         year = 1984,
        month = apr,
       volume = {279},
        pages = {596-609},
          doi = {10.1086/161924},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984ApJ...279..596Q},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{Malin80,
       author = {{Malin}, D.~F. and {Carter}, D.},
        title = "{Giant shells around normal elliptical galaxies}",
      journal = {NAT},
     keywords = {Astronomical Photography, Elliptical Galaxies, Galactic Evolution, Intergalactic Media, Photointerpretation, Brightness, Schmidt Telescopes, Astrophysics},
         year = 1980,
        month = jun,
       volume = {285},
       number = {5767},
        pages = {643-645},
          doi = {10.1038/285643a0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980Natur.285..643M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{martin22,
       author = {{Martin}, G. and {Bazkiaei}, A.~E. and {Spavone}, M. and {Iodice}, E. and {Mihos}, J.~C. and {Montes}, M. and {Benavides}, J.~A. and {Brough}, S. and {Carlin}, J.~L. and {Collins}, C.~A. and {Duc}, P.~A. and {G{\'o}mez}, F.~A. and {Galaz}, G. and {Hern{\'a}ndez-Toledo}, H.~M. and {Jackson}, R.~A. and {Kaviraj}, S. and {Knapen}, J.~H. and {Mart{\'\i}nez-Lombilla}, C. and {McGee}, S. and {O'Ryan}, D. and {Prole}, D.~J. and {Rich}, R.~M. and {Rom{\'a}n}, J. and {Shah}, E.~A. and {Starkenburg}, T.~K. and {Watkins}, A.~E. and {Zaritsky}, D. and {Pichon}, C. and {Armus}, L. and {Bianconi}, M. and {Buitrago}, F. and {Bus{\'a}}, I. and {Davis}, F. and {Demarco}, R. and {Desmons}, A. and {Garc{\'\i}a}, P. and {Graham}, A.~W. and {Holwerda}, B. and {Hon}, D.~S. -H. and {Khalid}, A. and {Klehammer}, J. and {Klutse}, D.~Y. and {Lazar}, I. and {Nair}, P. and {Noakes-Kettel}, E.~A. and {Rutkowski}, M. and {Saha}, K. and {Sahu}, N. and {Sola}, E. and {V{\'a}zquez-Mata}, J.~A. and {Vera-Casanova}, A. and {Yoon}, I.},
        title = "{Preparing for low surface brightness science with the Vera C. Rubin Observatory: Characterization of tidal features from mock images}",
      journal = {MNRAS},
     keywords = {methods: numerical, galaxies: interactions, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = jun,
       volume = {513},
       number = {1},
        pages = {1459-1487},
          doi = {10.1093/mnras/stac1003},
archivePrefix = {arXiv},
       eprint = {2203.07675},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.513.1459M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{fall80,
       author = {{Fall}, S.~M. and {Efstathiou}, G.},
        title = "{Formation and rotation of disc galaxies with haloes.}",
      journal = {MNRAS},
     keywords = {Disk Galaxies, Galactic Evolution, Galactic Rotation, Galactic Structure, Halos, Angular Momentum, Astronomical Models, Interstellar Gas, Mass Ratios, Astrophysics},
         year = 1980,
        month = oct,
       volume = {193},
        pages = {189-206},
          doi = {10.1093/mnras/193.2.189},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980MNRAS.193..189F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{bosch02,
       author = {{van den Bosch}, Frank C. and {Abel}, Tom and {Croft}, Rupert A.~C. and {Hernquist}, Lars and {White}, Simon D.~M.},
        title = "{The Angular Momentum of Gas in Protogalaxies. I. Implications for the Formation of Disk Galaxies}",
      journal = {APJ},
     keywords = {Cosmology: Dark Matter, Galaxies: Formation, Galaxies: Halos, Galaxies: Structure, Methods: n-Body Simulations, Astrophysics},
         year = 2002,
        month = sep,
       volume = {576},
       number = {1},
        pages = {21-35},
          doi = {10.1086/341619},
archivePrefix = {arXiv},
       eprint = {astro-ph/0201095},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...576...21V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{agertz11,
       author = {{Agertz}, Oscar and {Teyssier}, Romain and {Moore}, Ben},
        title = "{The formation of disc galaxies in a {\ensuremath{\Lambda}}CDM universe}",
      journal = {MNRAS},
     keywords = {methods: numerical, galaxies: evolution, galaxies: formation, galaxies: haloes, galaxies: spiral, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = jan,
       volume = {410},
       number = {2},
        pages = {1391-1408},
          doi = {10.1111/j.1365-2966.2010.17530.x},
archivePrefix = {arXiv},
       eprint = {1004.0005},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.410.1391A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{martinez24,
       author = {{Mart{\'\i}nez-Delgado}, David and {Roca-F{\`a}brega}, Santi and {Gil de Paz}, Armando and {Erkal}, Denis and {Mir{\'o}-Carretero}, Juan and {Makarov}, Dmitry and {Voggel}, Karina T. and {Leaman}, Ryan and {Boschin}, Walter and {Pearson}, Sarah and {Donatiello}, Giuseppe and {Rubtsov}, Evgenii and {Akhlaghi}, Mohammad and {Gomez-Flechoso}, M. Angeles and {Raji}, Samane and {Lang}, Dustin and {Block}, Adam and {Gallego}, Jesus and {Carrasco}, Esperanza and {Garc{\'\i}a-Vargas}, Mar{\'\i}a Luisa and {Iglesias-P{\'a}ramo}, Jorge and {Pascual}, Sergio and {Cardiel}, Nicolas and {P{\'e}rez-Calpena}, Ana and {Castillo-Morales}, Africa and {G{\'o}mez-Alvarez}, Pedro},
        title = "{Once in a blue stream. Detection of recent star formation in the NGC 7241 stellar stream with MEGARA}",
      journal = {AAP},
     keywords = {galaxies: dwarf, galaxies: formation, galaxies: interactions, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2024,
        month = apr,
       volume = {684},
          eid = {A157},
        pages = {A157},
          doi = {10.1051/0004-6361/202244350},
archivePrefix = {arXiv},
       eprint = {2112.07029},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A&A...684A.157M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{laine24,
       author = {{Laine}, Seppo and {Mart{\'\i}nez-Delgado}, David and {Webb}, Kristi A. and {Akhlaghi}, Mohammad and {Baena-Gall{\'e}}, Roberto and {Paudel}, Sanjaya and {Stein}, Michael and {Erkal}, Denis},
        title = "{Stellar Population Properties in the Stellar Streams around SPRC047}",
      journal = {APJ},
     keywords = {Stellar streams, Tidal disruption, Galaxy mergers, Galaxy evolution, Astronomy image processing, Spectral energy distribution, 2166, 1696, 608, 594, 2306, 2129, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = feb,
       volume = {962},
       number = {2},
          eid = {111},
        pages = {111},
          doi = {10.3847/1538-4357/ad16e4},
archivePrefix = {arXiv},
       eprint = {2312.05358},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024ApJ...962..111L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{javanmardi16,
       author = {{Javanmardi}, B. and {Martinez-Delgado}, D. and {Kroupa}, P. and {Henkel}, C. and {Crawford}, K. and {Teuwen}, K. and {Gabany}, R.~J. and {Hanson}, M. and {Chonis}, T.~S. and {Neyer}, F.},
        title = "{DGSAT: Dwarf Galaxy Survey with Amateur Telescopes. I. Discovery of low surface brightness systems around nearby spiral galaxies}",
      journal = {AAP},
     keywords = {galaxies: dwarf, galaxies: formation, galaxies: fundamental parameters, galaxies: statistics, galaxies: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = apr,
       volume = {588},
          eid = {A89},
        pages = {A89},
          doi = {10.1051/0004-6361/201527745},
archivePrefix = {arXiv},
       eprint = {1511.04446},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...588A..89J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{infante24,
       author = {{Infante-Sainz}, Ra{\'u}l and {Akhlaghi}, Mohammad},
        title = "{Gnuastro: Visualizing the Full Dynamic Range in Color Images}",
      journal = {RNAAS},
     keywords = {Astronomy software, Astronomy data visualization, Open source software, Low surface brightness galaxies, 1855, 1968, 1866, 940, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies, Computer Science - Computer Vision and Pattern Recognition},
         year = 2024,
        month = jan,
       volume = {8},
       number = {1},
          eid = {10},
        pages = {10},
          doi = {10.3847/2515-5172/ad1aae},
archivePrefix = {arXiv},
       eprint = {2401.03814},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024RNAAS...8...10I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{cherinka19,
       author = {{Cherinka}, Brian and {Andrews}, Brett H. and
         {S{\'a}nchez-Gallego}, Jos{\'e} and {Brownstein}, Joel and
         {Argudo-Fern{\'a}ndez}, Mar{\'\i}a and {Blanton}, Michael and
         {Bundy}, Kevin and {Jones}, Amy and {Masters}, Karen and
         {Law}, David R. and {Rowlands}, Kate and {Weijmans}, Anne-Marie and
         {Westfall}, Kyle and {Yan}, Renbin},
        title = "{Marvin: A Tool Kit for Streamlined Access and Visualization of the SDSS-IV MaNGA Data Set}",
      journal = {AJ},
     keywords = {astronomical databases: miscellaneous, methods: data analysis, surveys, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Aug",
       volume = {158},
       number = {2},
          eid = {74},
        pages = {74},
          doi = {10.3847/1538-3881/ab2634},
archivePrefix = {arXiv},
       eprint = {1812.03833},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....158...74C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{bonoli21,
       author = {{Bonoli}, S. and {Mar{\'\i}n-Franch}, A. and {Varela}, J. and {V{\'a}zquez Rami{\'o}}, H. and {Abramo}, L.~R. and {Cenarro}, A.~J. and {Dupke}, R.~A. and {V{\'\i}lchez}, J.~M. and {Crist{\'o}bal-Hornillos}, D. and {Gonz{\'a}lez Delgado}, R.~M. and {Hern{\'a}ndez-Monteagudo}, C. and {L{\'o}pez-Sanjuan}, C. and {Muniesa}, D.~J. and {Civera}, T. and {Ederoclite}, A. and {Hern{\'a}n-Caballero}, A. and {Marra}, V. and {Baqui}, P.~O. and {Cortesi}, A. and {Cypriano}, E.~S. and {Daflon}, S. and {de Amorim}, A.~L. and {D{\'\i}az-Garc{\'\i}a}, L.~A. and {Diego}, J.~M. and {Mart{\'\i}nez-Solaeche}, G. and {P{\'e}rez}, E. and {Placco}, V.~M. and {Prada}, F. and {Queiroz}, C. and {Alcaniz}, J. and {Alvarez-Candal}, A. and {Cepa}, J. and {Maroto}, A.~L. and {Roig}, F. and {Siffert}, B.~B. and {Taylor}, K. and {Benitez}, N. and {Moles}, M. and {Sodr{\'e}}, L. and {Carneiro}, S. and {Mendes de Oliveira}, C. and {Abdalla}, E. and {Angulo}, R.~E. and {Aparicio Resco}, M. and {Balaguera-Antol{\'\i}nez}, A. and {Ballesteros}, F.~J. and {Brito-Silva}, D. and {Broadhurst}, T. and {Carrasco}, E.~R. and {Castro}, T. and {Cid Fernandes}, R. and {Coelho}, P. and {de Melo}, R.~B. and {Doubrawa}, L. and {Fernandez-Soto}, A. and {Ferrari}, F. and {Finoguenov}, A. and {Garc{\'\i}a-Benito}, R. and {Iglesias-P{\'a}ramo}, J. and {Jim{\'e}nez-Teja}, Y. and {Kitaura}, F.~S. and {Laur}, J. and {Lopes}, P.~A.~A. and {Lucatelli}, G. and {Mart{\'\i}nez}, V.~J. and {Maturi}, M. and {Overzier}, R.~A. and {Pigozzo}, C. and {Quartin}, M. and {Rodr{\'\i}guez-Mart{\'\i}n}, J.~E. and {Salzano}, V. and {Tamm}, A. and {Tempel}, E. and {Umetsu}, K. and {Valdivielso}, L. and {von Marttens}, R. and {Zitrin}, A. and {D{\'\i}az-Mart{\'\i}n}, M.~C. and {L{\'o}pez-Alegre}, G. and {L{\'o}pez-Sainz}, A. and {Yanes-D{\'\i}az}, A. and {Rueda-Teruel}, F. and {Rueda-Teruel}, S. and {Abril Iba{\~n}ez}, J. and {L Ant{\'o}n Bravo}, J. and {Bello Ferrer}, R. and {Bielsa}, S. and {Casino}, J.~M. and {Castillo}, J. and {Chueca}, S. and {Cuesta}, L. and {Garzar{\'a}n Calderaro}, J. and {Iglesias-Marzoa}, R. and {{\'I}niguez}, C. and {Lamadrid Gutierrez}, J.~L. and {Lopez-Martinez}, F. and {Lozano-P{\'e}rez}, D. and {Ma{\'\i}cas Sacrist{\'a}n}, N. and {Molina-Ib{\'a}{\~n}ez}, E.~L. and {Moreno-Signes}, A. and {Rodr{\'\i}guez Llano}, S. and {Royo Navarro}, M. and {Tilve Rua}, V. and {Andrade}, U. and {Alfaro}, E.~J. and {Akras}, S. and {Arnalte-Mur}, P. and {Ascaso}, B. and {Barbosa}, C.~E. and {Beltr{\'a}n Jim{\'e}nez}, J. and {Benetti}, M. and {Bengaly}, C.~A.~P. and {Bernui}, A. and {Blanco-Pillado}, J.~J. and {Borges Fernandes}, M. and {Bregman}, J.~N. and {Bruzual}, G. and {Calderone}, G. and {Carvano}, J.~M. and {Casarini}, L. and {Chaves-Montero}, J. and {Chies-Santos}, A.~L. and {Coutinho de Carvalho}, G. and {Dimauro}, P. and {Duarte Puertas}, S. and {Figueruelo}, D. and {Gonz{\'a}lez-Serrano}, J.~I. and {Guerrero}, M.~A. and {Gurung-L{\'o}pez}, S. and {Herranz}, D. and {Huertas-Company}, M. and {Irwin}, J.~A. and {Izquierdo-Villalba}, D. and {Kanaan}, A. and {Kehrig}, C. and {Kirkpatrick}, C.~C. and {Lim}, J. and {Lopes}, A.~R. and {Lopes de Oliveira}, R. and {Marcos-Caballero}, A. and {Mart{\'\i}nez-Delgado}, D. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Mart{\'\i}nez-Somonte}, G. and {Oliveira}, N. and {Orsi}, A.~A. and {Penna-Lima}, M. and {Reis}, R.~R.~R. and {Spinoso}, D. and {Tsujikawa}, S. and {Vielva}, P. and {Vitorelli}, A.~Z. and {Xia}, J.~Q. and {Yuan}, H.~B. and {Arroyo-Polonio}, A. and {Dantas}, M.~L.~L. and {Galarza}, C.~A. and {Gon{\c{c}}alves}, D.~R. and {Gon{\c{c}}alves}, R.~S. and {Gonzalez}, J.~E. and {Gonzalez}, A.~H. and {Greisel}, N. and {Jim{\'e}nez-Esteban}, F. and {Landim}, R.~G. and {Lazzaro}, D. and {Magris}, G. and {Monteiro-Oliveira}, R. and {Pereira}, C.~B. and {Rebou{\c{c}}as}, M.~J. and {Rodriguez-Espinosa}, J.~M. and {Santos da Costa}, S. and {Telles}, E.},
        title = "{The miniJPAS survey: A preview of the Universe in 56 colors}",
      journal = {AAP},
     keywords = {surveys, techniques: photometric, astronomical databases: miscellaneous, stars: general, galaxies: general, cosmology: observations, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = sep,
       volume = {653},
          eid = {A31},
        pages = {A31},
          doi = {10.1051/0004-6361/202038841},
archivePrefix = {arXiv},
       eprint = {2007.01910},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...653A..31B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{akhlaghi19b,
       author = {{Akhlaghi}, Mohammad},
        title = "{Separating Detection and Catalog Production}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
    booktitle = {Astronomical Data Analysis Software and Systems XXVI},
         year = 2019,
       editor = {{Molinaro}, Marco and {Shortridge}, Keith and {Pasian}, Fabio},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {521},
        month = oct,
        pages = {299},
          doi = {10.48550/arXiv.1611.06387},
archivePrefix = {arXiv},
       eprint = {1611.06387},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ASPC..521..299A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}










@ARTICLE{bundy15,
       author = {{Bundy}, Kevin and {Bershady}, Matthew A. and {Law}, David R. and {Yan}, Renbin and {Drory}, Niv and {MacDonald}, Nicholas and {Wake}, David A. and {Cherinka}, Brian and {S{\'a}nchez-Gallego}, Jos{\'e} R. and {Weijmans}, Anne-Marie and {Thomas}, Daniel and {Tremonti}, Christy and {Masters}, Karen and {Coccato}, Lodovico and {Diamond-Stanic}, Aleksandar M. and {Arag{\'o}n-Salamanca}, Alfonso and {Avila-Reese}, Vladimir and {Badenes}, Carles and {Falc{\'o}n-Barroso}, J{\'e}sus and {Belfiore}, Francesco and {Bizyaev}, Dmitry and {Blanc}, Guillermo A. and {Bland-Hawthorn}, Joss and {Blanton}, Michael R. and {Brownstein}, Joel R. and {Byler}, Nell and {Cappellari}, Michele and {Conroy}, Charlie and {Dutton}, Aaron A. and {Emsellem}, Eric and {Etherington}, James and {Frinchaboy}, Peter M. and {Fu}, Hai and {Gunn}, James E. and {Harding}, Paul and {Johnston}, Evelyn J. and {Kauffmann}, Guinevere and {Kinemuchi}, Karen and {Klaene}, Mark A. and {Knapen}, Johan H. and {Leauthaud}, Alexie and {Li}, Cheng and {Lin}, Lihwai and {Maiolino}, Roberto and {Malanushenko}, Viktor and {Malanushenko}, Elena and {Mao}, Shude and {Maraston}, Claudia and {McDermid}, Richard M. and {Merrifield}, Michael R. and {Nichol}, Robert C. and {Oravetz}, Daniel and {Pan}, Kaike and {Parejko}, John K. and {Sanchez}, Sebastian F. and {Schlegel}, David and {Simmons}, Audrey and {Steele}, Oliver and {Steinmetz}, Matthias and {Thanjavur}, Karun and {Thompson}, Benjamin A. and {Tinker}, Jeremy L. and {van den Bosch}, Remco C.~E. and {Westfall}, Kyle B. and {Wilkinson}, David and {Wright}, Shelley and {Xiao}, Ting and {Zhang}, Kai},
        title = "{Overview of the SDSS-IV MaNGA Survey: Mapping nearby Galaxies at Apache Point Observatory}",
      journal = {APJ},
     keywords = {galaxies: evolution, galaxies: general, surveys, techniques: imaging spectroscopy, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = jan,
       volume = {798},
       number = {1},
          eid = {7},
        pages = {7},
          doi = {10.1088/0004-637X/798/1/7},
archivePrefix = {arXiv},
       eprint = {1412.1482},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...798....7B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{martinez23,
       author = {{Mart{\'\i}nez-Delgado}, David and {Cooper}, Andrew P. and {Rom{\'a}n}, Javier and {Pillepich}, Annalisa and {Erkal}, Denis and {Pearson}, Sarah and {Moustakas}, John and {Laporte}, Chervin F.~P. and {Laine}, Seppo and {Akhlaghi}, Mohammad and {Lang}, Dustin and {Makarov}, Dmitry and {Borlaff}, Alejandro S. and {Donatiello}, Giuseppe and {Pearson}, William J. and {Mir{\'o}-Carretero}, Juan and {Cuillandre}, Jean-Charles and {Dom{\'\i}nguez}, Helena and {Roca-F{\`a}brega}, Santi and {Frenk}, Carlos S. and {Schmidt}, Judy and {G{\'o}mez-Flechoso}, Mar{\'\i}a A. and {Guzman}, Rafael and {Libeskind}, Noam I. and {Dey}, Arjun and {Weaver}, Benjamin A. and {Schlegel}, David and {Myers}, Adam D. and {Valdes}, Frank G.},
        title = "{Hidden depths in the local Universe: The Stellar Stream Legacy Survey}",
      journal = {AAP},
     keywords = {galaxies: interactions, galaxies: dwarf, galaxies: formation, surveys, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = mar,
       volume = {671},
          eid = {A141},
        pages = {A141},
          doi = {10.1051/0004-6361/202245011},
archivePrefix = {arXiv},
       eprint = {2104.06071},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...671A.141M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{kathryn01,
       author = {{Johnston}, Kathryn V. and {Sackett}, Penny D. and {Bullock}, James S.},
        title = "{Interpreting Debris from Satellite Disruption in External Galaxies}",
      journal = {APJ},
     keywords = {Cosmology: Dark Matter, Galaxies: Evolution, Galaxies: Formation, Galaxies: Halos, galaxies: individual (M31, M32, NGC 205, NGC 5907), Galaxies: Kinematics and Dynamics, Galaxies: Local Group, Astrophysics},
         year = 2001,
        month = aug,
       volume = {557},
       number = {1},
        pages = {137-149},
          doi = {10.1086/321644},
archivePrefix = {arXiv},
       eprint = {astro-ph/0101543},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...557..137J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{desi24,
       author = {{DESI Collaboration} and {Adame}, A.~G. and {Aguilar}, J. and {Ahlen}, S. and {Alam}, S. and {Aldering}, G. and {Alexander}, D.~M. and {Alfarsy}, R. and {Allende Prieto}, C. and {Alvarez}, M. and {Alves}, O. and {Anand}, A. and {Andrade-Oliveira}, F. and {Armengaud}, E. and {Asorey}, J. and {Avila}, S. and {Aviles}, A. and {Bailey}, S. and {Balaguera-Antol{\'\i}nez}, A. and {Ballester}, O. and {Baltay}, C. and {Bault}, A. and {Bautista}, J. and {Behera}, J. and {Beltran}, S.~F. and {BenZvi}, S. and {Beraldo e Silva}, L. and {Bermejo-Climent}, J.~R. and {Berti}, A. and {Besuner}, R. and {Beutler}, F. and {Bianchi}, D. and {Blake}, C. and {Blum}, R. and {Bolton}, A.~S. and {Brieden}, S. and {Brodzeller}, A. and {Brooks}, D. and {Brown}, Z. and {Buckley-Geer}, E. and {Burtin}, E. and {Cabayol-Garcia}, L. and {Cai}, Z. and {Canning}, R. and {Cardiel-Sas}, L. and {Carnero Rosell}, A. and {Castander}, F.~J. and {Cervantes-Cota}, J.~L. and {Chabanier}, S. and {Chaussidon}, E. and {Chaves-Montero}, J. and {Chen}, S. and {Chen}, X. and {Chuang}, C. and {Claybaugh}, T. and {Cole}, S. and {Cooper}, A.~P. and {Cuceu}, A. and {Davis}, T.~M. and {Dawson}, K. and {de Belsunce}, R. and {de la Cruz}, R. and {de la Macorra}, A. and {Della Costa}, J. and {de Mattia}, A. and {Demina}, R. and {Demirbozan}, U. and {DeRose}, J. and {Dey}, A. and {Dey}, B. and {Dhungana}, G. and {Ding}, J. and {Ding}, Z. and {Doel}, P. and {Doshi}, R. and {Douglass}, K. and {Edge}, A. and {Eftekharzadeh}, S. and {Eisenstein}, D.~J. and {Elliott}, A. and {Ereza}, J. and {Escoffier}, S. and {Fagrelius}, P. and {Fan}, X. and {Fanning}, K. and {Fawcett}, V.~A. and {Ferraro}, S. and {Flaugher}, B. and {Font-Ribera}, A. and {Forero-Romero}, J.~E. and {Forero-S{\'a}nchez}, D. and {Frenk}, C.~S. and {G{\"a}nsicke}, B.~T. and {Garc{\'\i}a}, L. {\'A}. and {Garc{\'\i}a-Bellido}, J. and {Garcia-Quintero}, C. and {Garrison}, L.~H. and {Gil-Mar{\'\i}n}, H. and {Golden-Marx}, J. and {Gontcho A Gontcho}, S. and {Gonzalez-Morales}, A.~X. and {Gonzalez-Perez}, V. and {Gordon}, C. and {Graur}, O. and {Green}, D. and {Gruen}, D. and {Guy}, J. and {Hadzhiyska}, B. and {Hahn}, C. and {Han}, J.~J. and {Hanif}, M.~M.~S. and {Herrera-Alcantar}, H.~K. and {Honscheid}, K. and {Hou}, J. and {Howlett}, C. and {Huterer}, D. and {Ir{\v{s}}i{\v{c}}}, V. and {Ishak}, M. and {Jacques}, A. and {Jana}, A. and {Jiang}, L. and {Jimenez}, J. and {Jing}, Y.~P. and {Joudaki}, S. and {Joyce}, R. and {Jullo}, E. and {Juneau}, S. and {Kara{\c{c}}ayl{\i}}, N.~G. and {Karim}, T. and {Kehoe}, R. and {Kent}, S. and {Khederlarian}, A. and {Kim}, S. and {Kirkby}, D. and {Kisner}, T. and {Kitaura}, F. and {Kizhuprakkat}, N. and {Kneib}, J. and {Koposov}, S.~E. and {Kov{\'a}cs}, A. and {Kremin}, A. and {Krolewski}, A. and {L'Huillier}, B. and {Lahav}, O. and {Lambert}, A. and {Lamman}, C. and {Lan}, T. -W. and {Landriau}, M. and {Lang}, D. and {Lange}, J.~U. and {Lasker}, J. and {Leauthaud}, A. and {Le Guillou}, L. and {Levi}, M.~E. and {Li}, T.~S. and {Linder}, E. and {Lyons}, A. and {Magneville}, C. and {Manera}, M. and {Manser}, C.~J. and {Margala}, D. and {Martini}, P. and {McDonald}, P. and {Medina}, G.~E. and {Medina-Varela}, L. and {Meisner}, A. and {Mena-Fern{\'a}ndez}, J. and {Meneses-Rizo}, J. and {Mezcua}, M. and {Miquel}, R. and {Montero-Camacho}, P. and {Moon}, J. and {Moore}, S. and {Moustakas}, J. and {Mueller}, E. and {Mundet}, J. and {Mu{\~n}oz-Guti{\'e}rrez}, A. and {Myers}, A.~D. and {Nadathur}, S. and {Napolitano}, L. and {Neveux}, R. and {Newman}, J.~A. and {Nie}, J. and {Nikutta}, R. and {Niz}, G. and {Norberg}, P. and {Noriega}, H.~E. and {Paillas}, E. and {Palanque-Delabrouille}, N. and {Palmese}, A. and {Pan}, Z. and {Parkinson}, D. and {Penmetsa}, S. and {Percival}, W.~J. and {P{\'e}rez-Fern{\'a}ndez}, A. and {P{\'e}rez-R{\`a}fols}, I. and {Pieri}, M. and {Poppett}, C. and {Porredon}, A. and {Pothier}, S. and {Prada}, F. and {Pucha}, R. and {Raichoor}, A. and {Ram{\'\i}rez-P{\'e}rez}, C. and {Ramirez-Solano}, S. and {Rashkovetskyi}, M. and {Ravoux}, C. and {Rocher}, A. and {Rockosi}, C. and {Ross}, A.~J. and {Rossi}, G. and {Ruggeri}, R. and {Ruhlmann-Kleider}, V. and {Sabiu}, C.~G. and {Said}, K. and {Saintonge}, A. and {Samushia}, L. and {Sanchez}, E. and {Saulder}, C. and {Schaan}, E. and {Schlafly}, E.~F. and {Schlegel}, D. and {Scholte}, D. and {Schubnell}, M. and {Seo}, H. and {Shafieloo}, A. and {Sharples}, R. and {Sheu}, W. and {Silber}, J. and {Sinigaglia}, F. and {Siudek}, M. and {Slepian}, Z. and {Smith}, A. and {Soumagnac}, M.~T. and {Sprayberry}, D. and {Stephey}, L. and {Su{\'a}rez-P{\'e}rez}, J. and {Sun}, Z. and {Tan}, T. and {Tarl{\'e}}, G. and {Tojeiro}, R. and {Ure{\~n}a-L{\'o}pez}, L.~A. and {Vaisakh}, R. and {Valcin}, D. and {Valdes}, F. and {Valluri}, M. and {Vargas-Maga{\~n}a}, M. and {Variu}, A. and {Verde}, L. and {Walther}, M. and {Wang}, B. and {Wang}, M.~S. and {Weaver}, B.~A. and {Weaverdyck}, N. and {Wechsler}, R.~H. and {White}, M. and {Xie}, Y. and {Yang}, J. and {Y{\`e}che}, C. and {Yu}, J. and {Yuan}, S. and {Zhang}, H. and {Zhang}, Z. and {Zhao}, C. and {Zheng}, Z. and {Zhou}, R. and {Zhou}, Z. and {Zou}, H. and {Zou}, S. and {Zu}, Y.},
        title = "{The Early Data Release of the Dark Energy Spectroscopic Instrument}",
      journal = {AJ},
     keywords = {Astronomy data reduction, Observational cosmology, Astronomy databases, Astronomy data analysis, Astronomy software, Surveys, Redshift surveys, 1861, 1146, 83, 1858, 1855, 1671, 1378, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2024,
        month = aug,
       volume = {168},
       number = {2},
          eid = {58},
        pages = {58},
          doi = {10.3847/1538-3881/ad3217},
archivePrefix = {arXiv},
       eprint = {2306.06308},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024AJ....168...58D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{heckman90,
       author = {{Heckman}, Timothy M. and {Armus}, Lee and {Miley}, George K.},
        title = "{On the Nature and Implications of Starburst-driven Galactic Superwinds}",
      journal = {APJS},
     keywords = {Far Infrared Radiation, Interstellar Gas, Starburst Galaxies, Stellar Winds, Galactic Structure, Intergalactic Media, Nebulae, Optical Emission Spectroscopy, Stellar Motions, Astrophysics, GALAXIES: INTERGALACTIC MEDIUM, GALAXIES: INTERNAL MOTIONS, GALAXIES: INTERSTELLAR MATTER, GALAXIES: STRUCTURE, INFRARED: SOURCES},
         year = 1990,
        month = dec,
       volume = {74},
        pages = {833},
          doi = {10.1086/191522},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990ApJS...74..833H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{veilleux05,
       author = {{Veilleux}, Sylvain and {Cecil}, Gerald and {Bland-Hawthorn}, Joss},
        title = "{Galactic Winds}",
      journal = {ARAA},
     keywords = {Astrophysics},
         year = 2005,
        month = sep,
       volume = {43},
       number = {1},
        pages = {769-826},
          doi = {10.1146/annurev.astro.43.072103.150610},
archivePrefix = {arXiv},
       eprint = {astro-ph/0504435},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ARA&A..43..769V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{chrisJ09,
       author = {{Lintott}, Chris J. and {Schawinski}, Kevin and {Keel}, William and {van Arkel}, Hanny and {Bennert}, Nicola and {Edmondson}, Edward and {Thomas}, Daniel and {Smith}, Daniel J.~B. and {Herbert}, Peter D. and {Jarvis}, Matt J. and {Virani}, Shanil and {Andreescu}, Dan and {Bamford}, Steven P. and {Land}, Kate and {Murray}, Phil and {Nichol}, Robert C. and {Raddick}, M. Jordan and {Slosar}, An{\v{z}}e and {Szalay}, Alex and {Vandenberg}, Jan},
        title = "{Galaxy Zoo: `Hanny's Voorwerp', a quasar light echo?}",
      journal = {MNRAS},
     keywords = {galaxies: active, galaxies: individual: IC2497, galaxies: peculiar, quasars: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2009,
        month = oct,
       volume = {399},
       number = {1},
        pages = {129-140},
          doi = {10.1111/j.1365-2966.2009.15299.x},
archivePrefix = {arXiv},
       eprint = {0906.5304},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.399..129L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{william24,
       author = {{Keel}, William C. and {Moiseev}, Alexei and {Uklein}, Roman and {Smirnova}, Aleksandrina},
        title = "{The TELPERION survey for extended emission regions around active galactic nuclei: a strongly interacting and merging galaxy sample}",
      journal = {MNRAS},
     keywords = {galaxies: active, galaxies: interactions, galaxies: Seyfert, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = may,
       volume = {530},
       number = {2},
        pages = {1624-1635},
          doi = {10.1093/mnras/stae946},
archivePrefix = {arXiv},
       eprint = {2403.04898},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024MNRAS.530.1624K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{moissev23,
       author = {{Moiseev}, Alexei V. and {Smirnova}, Aleksandrina A. and {Movsessian}, Tigran A.},
        title = "{Enigmatic Emission Structure around Mrk 783: Cross-Ionization of a Companion 100 kpc Away}",
      journal = {Universe},
     keywords = {galaxies:individual: Mrk 783, galaxies: active, galaxies: jets, galaxies: Seyfert, interstellar medium (ISM): nebulae, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = nov,
       volume = {9},
       number = {12},
          eid = {493},
        pages = {493},
          doi = {10.3390/universe9120493},
archivePrefix = {arXiv},
       eprint = {2311.12189},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023Univ....9..493M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{william22,
       author = {{Keel}, William C. and {Moiseev}, Alexei and {Kozlova}, D.~V. and {Ikhsanova}, A.~I. and {Oparin}, D.~V. and {Uklein}, R.~I. and {Smirnova}, A.~A. and {Eselevich}, M.~V.},
        title = "{The TELPERION survey for distant [O III] clouds around luminous and hibernating AGN}",
      journal = {MNRAS},
     keywords = {galaxies: active, galaxies: interactions, galaxies: Seyfert, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = mar,
       volume = {510},
       number = {3},
        pages = {4608-4625},
          doi = {10.1093/mnras/stab3656},
archivePrefix = {arXiv},
       eprint = {2112.07084},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.510.4608K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{schweizer13,
       author = {{Schweizer}, Fran{\c{c}}ois and {Seitzer}, Patrick and {Kelson}, Daniel D. and {Villanueva}, Edward V. and {Walth}, Gregory L.},
        title = "{The [O III] Nebula of the Merger Remnant NGC 7252: A Likely Faint Ionization Echo}",
      journal = {APJ},
     keywords = {galaxies: active, galaxies: evolution, galaxies: formation, galaxies: individual: NGC 7252, galaxies: interactions, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = aug,
       volume = {773},
       number = {2},
          eid = {148},
        pages = {148},
          doi = {10.1088/0004-637X/773/2/148},
archivePrefix = {arXiv},
       eprint = {1307.2233},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...773..148S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{toba14,
       author = {{Toba}, Y. and {Oyabu}, S. and {Matsuhara}, H. and {Malkan}, M.~A. and {Gandhi}, P. and {Nakagawa}, T. and {Isobe}, N. and {Shirahata}, M. and {Oi}, N. and {Ohyama}, Y. and {Takita}, S. and {Yamauchi}, C. and {Yano}, K.},
        title = "{Luminosity and Redshift Dependence of the Covering Factor of Active Galactic Nuclei viewed with WISE and Sloan Digital Sky Survey}",
      journal = {APJ},
     keywords = {catalogs, galaxies: active, galaxies: luminosity function, mass function, galaxies: nuclei, infrared: galaxies, methods: statistical, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = jun,
       volume = {788},
       number = {1},
          eid = {45},
        pages = {45},
          doi = {10.1088/0004-637X/788/1/45},
archivePrefix = {arXiv},
       eprint = {1404.4937},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...788...45T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{wenger00,
       author = {{Wenger}, M. and {Ochsenbein}, F. and {Egret}, D. and {Dubois}, P. and {Bonnarel}, F. and {Borde}, S. and {Genova}, F. and {Jasniewicz}, G. and {Lalo{\"e}}, S. and {Lesteven}, S. and {Monier}, R.},
        title = "{The SIMBAD astronomical database. The CDS reference database for astronomical objects}",
      journal = {AAPS},
     keywords = {ASTRONOMICAL DATA BASES: MISCELLANEOUS, CATALOGS, Astrophysics},
         year = 2000,
        month = apr,
       volume = {143},
        pages = {9-22},
          doi = {10.1051/aas:2000332},
archivePrefix = {arXiv},
       eprint = {astro-ph/0002110},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&AS..143....9W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@ARTICLE{keel12,
       author = {{Keel}, William C. and {Lintott}, Chris J. and {Schawinski}, Kevin and {Bennert}, Vardha N. and {Thomas}, Daniel and {Manning}, Anna and {Chojnowski}, S. Drew and {van Arkel}, Hanny and {Lynn}, Stuart},
        title = "{The History and Environment of a Faded Quasar: Hubble Space Telescope Observations of Hanny's Voorwerp and IC 2497}",
      journal = {AJ},
     keywords = {galaxies: active, galaxies: individual: IC 2497, quasars: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2012,
        month = aug,
       volume = {144},
       number = {2},
          eid = {66},
        pages = {66},
          doi = {10.1088/0004-6256/144/2/66},
archivePrefix = {arXiv},
       eprint = {1206.3797},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012AJ....144...66K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{zaragoza18,
       author = {{Zaragoza-Cardiel}, Javier and {Smith}, Beverly J. and {Rosado}, Margarita and {Beckman}, John E. and {Bitsakis}, Theodoros and {Camps-Fari{\~n}a}, Artemi and {Font}, Joan and {Cox}, Isaiah S.},
        title = "{Stellar Population Synthesis of Star-forming Clumps in Galaxy Pairs and Non-interacting Spiral Galaxies}",
      journal = {\apjs},
     keywords = {galaxies: fundamental parameters, galaxies: interactions, galaxies: photometry, galaxies: star formation, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = feb,
       volume = {234},
       number = {2},
          eid = {35},
        pages = {35},
          doi = {10.3847/1538-4365/aaa255},
archivePrefix = {arXiv},
       eprint = {1712.05408},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..234...35Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{weilbacher18,
       author = {{Weilbacher}, Peter M. and {Monreal-Ibero}, Ana and {Verhamme}, Anne and {Sandin}, Christer and {Steinmetz}, Matthias and {Kollatschny}, Wolfram and {Krajnovi{\'c}}, Davor and {Kamann}, Sebastian and {Roth}, Martin M. and {Erroz-Ferrer}, Santiago and {Marino}, Raffaella Anna and {Maseda}, Michael V. and {Wendt}, Martin and {Bacon}, Roland and {Dreizler}, Stefan and {Richard}, Johan and {Wisotzki}, Lutz},
        title = "{Lyman-continuum leakage as dominant source of diffuse ionized gas in the Antennae galaxy}",
      journal = {\aap},
     keywords = {galaxies: interactions, galaxies: individual: NGC 4038, NGC 4039, galaxies: ISM, ISM: structure, HII regions, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = apr,
       volume = {611},
          eid = {A95},
        pages = {A95},
          doi = {10.1051/0004-6361/201731669},
archivePrefix = {arXiv},
       eprint = {1712.04450},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...611A..95W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{zhou14,
       author = {{Zhou}, Zhi-Min and {Wu}, Hong and {Huang}, Lei and {Li}, Hong-Bin and {Zhou}, Zhi-Zhong and {Jia}, Jun-Jun and {Lam}, Man-I. and {Zhu}, Yi-Nan},
        title = "{Metallicity and star formation activities of the interacting system Arp 86 from observations with MOS on the Xinglong 2.16 m telescope}",
      journal = {Research in Astronomy and Astrophysics},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = nov,
       volume = {14},
       number = {11},
          eid = {1393-1405},
        pages = {1393-1405},
          doi = {10.1088/1674-4527/14/11/003},
archivePrefix = {arXiv},
       eprint = {1404.7037},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014RAA....14.1393Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{zhang20,
       author = {{Zhang}, Bing-qing and {Cao}, Chen and {Xu}, Cong K. and {Zhou}, Zhi-min and {Wu}, Hong},
        title = "{The Multi-object Spectroscopy Observation of Seven Interacting Galaxy Pairs: Metallicity Gradients and Star Formation Distributions}",
      journal = {\pasp},
     keywords = {galaxies: abundances, galaxies: evolution, galaxies: interactions, galaxies: star formation, Hii regions, techniques: spectroscopic},
         year = 2020,
        month = mar,
       volume = {132},
       number = {1009},
          eid = {034101},
        pages = {034101},
          doi = {10.1088/1538-3873/ab6714},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020PASP..132c4101Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{boquien19,
       author = {{Boquien}, M. and {Burgarella}, D. and {Roehlly}, Y. and {Buat}, V. and {Ciesla}, L. and {Corre}, D. and {Inoue}, A.~K. and {Salas}, H.},
        title = "{CIGALE: a python Code Investigating GALaxy Emission}",
      journal = {\aap},
     keywords = {methods: data analysis, methods: numerical, methods: statistical, galaxies: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = feb,
       volume = {622},
          eid = {A103},
        pages = {A103},
          doi = {10.1051/0004-6361/201834156},
archivePrefix = {arXiv},
       eprint = {1811.03094},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...622A.103B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{bell2003,
       author = {{Bell}, Eric F. and {McIntosh}, Daniel H. and {Katz}, Neal and {Weinberg}, Martin D.},
        title = "{The Optical and Near-Infrared Properties of Galaxies. I. Luminosity and Stellar Mass Functions}",
      journal = {\apjs},
     keywords = {Galaxies: Evolution, Galaxies: General, Galaxies: Luminosity Function, Mass Function, Galaxies: Stellar Content, Astrophysics},
         year = 2003,
        month = dec,
       volume = {149},
       number = {2},
        pages = {289-312},
          doi = {10.1086/378847},
archivePrefix = {arXiv},
       eprint = {astro-ph/0302543},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJS..149..289B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{willmer2018,
       author = {{Willmer}, Christopher N.~A.},
        title = "{The Absolute Magnitude of the Sun in Several Filters}",
      journal = {\apjs},
     keywords = {astronomical databases: miscellaneous, catalogs, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = jun,
       volume = {236},
       number = {2},
          eid = {47},
        pages = {47},
          doi = {10.3847/1538-4365/aabfdf},
archivePrefix = {arXiv},
       eprint = {1804.07788},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..236...47W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}









@ARTICLE{blanton17,
       author = {{Blanton}, Michael R. and {Bershady}, Matthew A. and {Abolfathi}, Bela and {Albareti}, Franco D. and {Allende Prieto}, Carlos and {Almeida}, Andres and {Alonso-Garc{\'\i}a}, Javier and {Anders}, Friedrich and {Anderson}, Scott F. and {Andrews}, Brett and {Aquino-Ort{\'\i}z}, Erik and {Arag{\'o}n-Salamanca}, Alfonso and {Argudo-Fern{\'a}ndez}, Maria and {Armengaud}, Eric and {Aubourg}, Eric and {Avila-Reese}, Vladimir and {Badenes}, Carles and {Bailey}, Stephen and {Barger}, Kathleen A. and {Barrera-Ballesteros}, Jorge and {Bartosz}, Curtis and {Bates}, Dominic and {Baumgarten}, Falk and {Bautista}, Julian and {Beaton}, Rachael and {Beers}, Timothy C. and {Belfiore}, Francesco and {Bender}, Chad F. and {Berlind}, Andreas A. and {Bernardi}, Mariangela and {Beutler}, Florian and {Bird}, Jonathan C. and {Bizyaev}, Dmitry and {Blanc}, Guillermo A. and {Blomqvist}, Michael and {Bolton}, Adam S. and {Boquien}, M{\'e}d{\'e}ric and {Borissova}, Jura and {van den Bosch}, Remco and {Bovy}, Jo and {Brandt}, William N. and {Brinkmann}, Jonathan and {Brownstein}, Joel R. and {Bundy}, Kevin and {Burgasser}, Adam J. and {Burtin}, Etienne and {Busca}, Nicol{\'a}s G. and {Cappellari}, Michele and {Delgado Carigi}, Maria Leticia and {Carlberg}, Joleen K. and {Carnero Rosell}, Aurelio and {Carrera}, Ricardo and {Chanover}, Nancy J. and {Cherinka}, Brian and {Cheung}, Edmond and {G{\'o}mez Maqueo Chew}, Yilen and {Chiappini}, Cristina and {Choi}, Peter Doohyun and {Chojnowski}, Drew and {Chuang}, Chia-Hsun and {Chung}, Haeun and {Cirolini}, Rafael Fernando and {Clerc}, Nicolas and {Cohen}, Roger E. and {Comparat}, Johan and {da Costa}, Luiz and {Cousinou}, Marie-Claude and {Covey}, Kevin and {Crane}, Jeffrey D. and {Croft}, Rupert A.~C. and {Cruz-Gonzalez}, Irene and {Garrido Cuadra}, Daniel and {Cunha}, Katia and {Damke}, Guillermo J. and {Darling}, Jeremy and {Davies}, Roger and {Dawson}, Kyle and {de la Macorra}, Axel and {Dell'Agli}, Flavia and {De Lee}, Nathan and {Delubac}, Timoth{\'e}e and {Di Mille}, Francesco and {Diamond-Stanic}, Aleks and {Cano-D{\'\i}az}, Mariana and {Donor}, John and {Downes}, Juan Jos{\'e} and {Drory}, Niv and {du Mas des Bourboux}, H{\'e}lion and {Duckworth}, Christopher J. and {Dwelly}, Tom and {Dyer}, Jamie and {Ebelke}, Garrett and {Eigenbrot}, Arthur D. and {Eisenstein}, Daniel J. and {Emsellem}, Eric and {Eracleous}, Mike and {Escoffier}, Stephanie and {Evans}, Michael L. and {Fan}, Xiaohui and {Fern{\'a}ndez-Alvar}, Emma and {Fernandez-Trincado}, J.~G. and {Feuillet}, Diane K. and {Finoguenov}, Alexis and {Fleming}, Scott W. and {Font-Ribera}, Andreu and {Fredrickson}, Alexander and {Freischlad}, Gordon and {Frinchaboy}, Peter M. and {Fuentes}, Carla E. and {Galbany}, Llu{\'\i}s and {Garcia-Dias}, R. and {Garc{\'\i}a-Hern{\'a}ndez}, D.~A. and {Gaulme}, Patrick and {Geisler}, Doug and {Gelfand}, Joseph D. and {Gil-Mar{\'\i}n}, H{\'e}ctor and {Gillespie}, Bruce A. and {Goddard}, Daniel and {Gonzalez-Perez}, Violeta and {Grabowski}, Kathleen and {Green}, Paul J. and {Grier}, Catherine J. and {Gunn}, James E. and {Guo}, Hong and {Guy}, Julien and {Hagen}, Alex and {Hahn}, ChangHoon and {Hall}, Matthew and {Harding}, Paul and {Hasselquist}, Sten and {Hawley}, Suzanne L. and {Hearty}, Fred and {Gonzalez Hern{\'a}ndez}, Jonay I. and {Ho}, Shirley and {Hogg}, David W. and {Holley-Bockelmann}, Kelly and {Holtzman}, Jon A. and {Holzer}, Parker H. and {Huehnerhoff}, Joseph and {Hutchinson}, Timothy A. and {Hwang}, Ho Seong and {Ibarra-Medel}, H{\'e}ctor J. and {da Silva Ilha}, Gabriele and {Ivans}, Inese I. and {Ivory}, KeShawn and {Jackson}, Kelly and {Jensen}, Trey W. and {Johnson}, Jennifer A. and {Jones}, Amy and {J{\"o}nsson}, Henrik and {Jullo}, Eric and {Kamble}, Vikrant and {Kinemuchi}, Karen and {Kirkby}, David and {Kitaura}, Francisco-Shu and {Klaene}, Mark and {Knapp}, Gillian R. and {Kneib}, Jean-Paul and {Kollmeier}, Juna A. and {Lacerna}, Ivan and {Lane}, Richard R. and {Lang}, Dustin and {Law}, David R. and {Lazarz}, Daniel and {Lee}, Youngbae and {Le Goff}, Jean-Marc and {Liang}, Fu-Heng and {Li}, Cheng and {Li}, Hongyu and {Lian}, Jianhui and {Lima}, Marcos and {Lin}, Lihwai and {Lin}, Yen-Ting and {Bertran de Lis}, Sara and {Liu}, Chao and {de Icaza Lizaola}, Miguel Angel C. and {Long}, Dan and {Lucatello}, Sara and {Lundgren}, Britt and {MacDonald}, Nicholas K. and {Deconto Machado}, Alice and {MacLeod}, Chelsea L. and {Mahadevan}, Suvrath and {Geimba Maia}, Marcio Antonio and {Maiolino}, Roberto and {Majewski}, Steven R. and {Malanushenko}, Elena and {Malanushenko}, Viktor and {Manchado}, Arturo and {Mao}, Shude and {Maraston}, Claudia and {Marques-Chaves}, Rui and {Masseron}, Thomas and {Masters}, Karen L. and {McBride}, Cameron K. and {McDermid}, Richard M. and {McGrath}, Brianne and {McGreer}, Ian D. and {Medina Pe{\~n}a}, Nicol{\'a}s and {Melendez}, Matthew},
        title = "{Sloan Digital Sky Survey IV: Mapping the Milky Way, Nearby Galaxies, and the Distant Universe}",
      journal = {\aj},
     keywords = {cosmology: observations, galaxies: general, Galaxy: general, instrumentation: spectrographs, stars: general, surveys, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = jul,
       volume = {154},
       number = {1},
          eid = {28},
        pages = {28},
          doi = {10.3847/1538-3881/aa7567},
archivePrefix = {arXiv},
       eprint = {1703.00052},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154...28B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@ARTICLE{balogh99,
       author = {{Balogh}, Michael L. and {Morris}, Simon L. and {Yee}, H.~K.~C. and {Carlberg}, R.~G. and {Ellingson}, Erica},
        title = "{Differential Galaxy Evolution in Cluster and Field Galaxies at z\raisebox{-0.5ex}\textasciitilde0.3}",
      journal = {\apj},
     keywords = {GALAXIES: CLUSTERS: GENERAL, GALAXIES: EVOLUTION, GALAXIES: PHOTOMETRY, GALAXIES: STELLAR CONTENT, Galaxies: Clusters: General, Galaxies: Evolution, Galaxies: Photometry, Galaxies: Stellar Content, Astrophysics},
         year = 1999,
        month = dec,
       volume = {527},
       number = {1},
        pages = {54-79},
          doi = {10.1086/308056},
archivePrefix = {arXiv},
       eprint = {astro-ph/9906470},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...527...54B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@ARTICLE{kauffmann03,
       author = {{Kauffmann}, Guinevere and {Heckman}, Timothy M. and {White}, Simon D.~M. and {Charlot}, St{\'e}phane and {Tremonti}, Christy and {Brinchmann}, Jarle and {Bruzual}, Gustavo and {Peng}, Eric W. and {Seibert}, Mark and {Bernardi}, Mariangela and {Blanton}, Michael and {Brinkmann}, Jon and {Castander}, Francisco and {Cs{\'a}bai}, Istvan and {Fukugita}, Masataka and {Ivezic}, Zeljko and {Munn}, Jeffrey A. and {Nichol}, Robert C. and {Padmanabhan}, Nikhil and {Thakar}, Aniruddha R. and {Weinberg}, David H. and {York}, Donald},
        title = "{Stellar masses and star formation histories for {}10$^{5}$ galaxies from the Sloan Digital Sky Survey}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: stellar content, Astrophysics},
         year = 2003,
        month = may,
       volume = {341},
       number = {1},
        pages = {33-53},
          doi = {10.1046/j.1365-8711.2003.06291.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0204055},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003MNRAS.341...33K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@ARTICLE{gallazzi05,
       author = {{Gallazzi}, Anna and {Charlot}, St{\'e}phane and {Brinchmann}, Jarle and {White}, Simon D.~M. and {Tremonti}, Christy A.},
        title = "{The ages and metallicities of galaxies in the local universe}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: stellar content, Astrophysics},
         year = 2005,
        month = sep,
       volume = {362},
       number = {1},
        pages = {41-58},
          doi = {10.1111/j.1365-2966.2005.09321.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0506539},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.362...41G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}









@ARTICLE{aihara19,
       author = {{Aihara}, Hiroaki and {AlSayyad}, Yusra and {Ando}, Makoto and {Armstrong}, Robert and {Bosch}, James and {Egami}, Eiichi and {Furusawa}, Hisanori and {Furusawa}, Junko and {Goulding}, Andy and {Harikane}, Yuichi and {Hikage}, Chiaki and {Ho}, Paul T.~P. and {Hsieh}, Bau-Ching and {Huang}, Song and {Ikeda}, Hiroyuki and {Imanishi}, Masatoshi and {Ito}, Kei and {Iwata}, Ikuru and {Jaelani}, Anton T. and {Kakuma}, Ryota and {Kawana}, Kojiro and {Kikuta}, Satoshi and {Kobayashi}, Umi and {Koike}, Michitaro and {Komiyama}, Yutaka and {Li}, Xiangchong and {Liang}, Yongming and {Lin}, Yen-Ting and {Luo}, Wentao and {Lupton}, Robert and {Lust}, Nate B. and {MacArthur}, Lauren A. and {Matsuoka}, Yoshiki and {Mineo}, Sogo and {Miyatake}, Hironao and {Miyazaki}, Satoshi and {More}, Surhud and {Murata}, Ryoma and {Namiki}, Shigeru V. and {Nishizawa}, Atsushi J. and {Oguri}, Masamune and {Okabe}, Nobuhiro and {Okamoto}, Sakurako and {Okura}, Yuki and {Ono}, Yoshiaki and {Onodera}, Masato and {Onoue}, Masafusa and {Osato}, Ken and {Ouchi}, Masami and {Shibuya}, Takatoshi and {Strauss}, Michael A. and {Sugiyama}, Naoshi and {Suto}, Yasushi and {Takada}, Masahiro and {Takagi}, Yuhei and {Takata}, Tadafumi and {Takita}, Satoshi and {Tanaka}, Masayuki and {Terai}, Tsuyoshi and {Toba}, Yoshiki and {Uchiyama}, Hisakazu and {Utsumi}, Yousuke and {Wang}, Shiang-Yu and {Wang}, Wenting and {Yamada}, Yoshihiko},
        title = "{Second data release of the Hyper Suprime-Cam Subaru Strategic Program}",
      journal = {\pasj},
     keywords = {astronomical databases: miscellaneous, cosmology: observations, galaxies: general, surveys, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = dec,
       volume = {71},
       number = {6},
          eid = {114},
        pages = {114},
          doi = {10.1093/pasj/psz103},
archivePrefix = {arXiv},
       eprint = {1905.12221},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASJ...71..114A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{petersson23,
       author = {{Petersson}, Jonathan and {Renaud}, Florent and {Agertz}, Oscar and {Dekel}, Avishai and {Duc}, Pierre-Alain},
        title = "{From starburst to quenching: merger-driven evolution of the star formation regimes in a shell galaxy}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: interactions, galaxies: starburst, galaxies: star formation, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = jan,
       volume = {518},
       number = {3},
        pages = {3261-3273},
          doi = {10.1093/mnras/stac3136},
archivePrefix = {arXiv},
       eprint = {2210.16333},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MNRAS.518.3261P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@INPROCEEDINGS{bacon10,
       author = {{Bacon}, R. and {Accardo}, M. and {Adjali}, L. and {Anwand}, H. and {Bauer}, S. and {Biswas}, I. and {Blaizot}, J. and {Boudon}, D. and {Brau-Nogue}, S. and {Brinchmann}, J. and {Caillier}, P. and {Capoani}, L. and {Carollo}, C.~M. and {Contini}, T. and {Couderc}, P. and {Daguis{\'e}}, E. and {Deiries}, S. and {Delabre}, B. and {Dreizler}, S. and {Dubois}, J. and {Dupieux}, M. and {Dupuy}, C. and {Emsellem}, E. and {Fechner}, T. and {Fleischmann}, A. and {Fran{\c{c}}ois}, M. and {Gallou}, G. and {Gharsa}, T. and {Glindemann}, A. and {Gojak}, D. and {Guiderdoni}, B. and {Hansali}, G. and {Hahn}, T. and {Jarno}, A. and {Kelz}, A. and {Koehler}, C. and {Kosmalski}, J. and {Laurent}, F. and {Le Floch}, M. and {Lilly}, S.~J. and {Lizon}, J. -L. and {Loupias}, M. and {Manescau}, A. and {Monstein}, C. and {Nicklas}, H. and {Olaya}, J. -C. and {Pares}, L. and {Pasquini}, L. and {P{\'e}contal-Rousset}, A. and {Pell{\'o}}, R. and {Petit}, C. and {Popow}, E. and {Reiss}, R. and {Remillieux}, A. and {Renault}, E. and {Roth}, M. and {Rupprecht}, G. and {Serre}, D. and {Schaye}, J. and {Soucail}, G. and {Steinmetz}, M. and {Streicher}, O. and {Stuik}, R. and {Valentin}, H. and {Vernet}, J. and {Weilbacher}, P. and {Wisotzki}, L. and {Yerle}, N.},
        title = "{The MUSE second-generation VLT instrument}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy III},
         year = 2010,
       editor = {{McLean}, Ian S. and {Ramsay}, Suzanne K. and {Takami}, Hideki},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {7735},
        month = jul,
          eid = {773508},
        pages = {773508},
          doi = {10.1117/12.856027},
archivePrefix = {arXiv},
       eprint = {2211.16795},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010SPIE.7735E..08B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{sanchez12,
       author = {{S{\'a}nchez}, S.~F. and {Kennicutt}, R.~C. and {Gil de Paz}, A. and {van de Ven}, G. and {V{\'\i}lchez}, J.~M. and {Wisotzki}, L. and {Walcher}, C.~J. and {Mast}, D. and {Aguerri}, J.~A.~L. and {Albiol-P{\'e}rez}, S. and {Alonso-Herrero}, A. and {Alves}, J. and {Bakos}, J. and {Bart{\'a}kov{\'a}}, T. and {Bland-Hawthorn}, J. and {Boselli}, A. and {Bomans}, D.~J. and {Castillo-Morales}, A. and {Cortijo-Ferrero}, C. and {de Lorenzo-C{\'a}ceres}, A. and {Del Olmo}, A. and {Dettmar}, R. -J. and {D{\'\i}az}, A. and {Ellis}, S. and {Falc{\'o}n-Barroso}, J. and {Flores}, H. and {Gallazzi}, A. and {Garc{\'\i}a-Lorenzo}, B. and {Gonz{\'a}lez Delgado}, R. and {Gruel}, N. and {Haines}, T. and {Hao}, C. and {Husemann}, B. and {Igl{\'e}sias-P{\'a}ramo}, J. and {Jahnke}, K. and {Johnson}, B. and {Jungwiert}, B. and {Kalinova}, V. and {Kehrig}, C. and {Kupko}, D. and {L{\'o}pez-S{\'a}nchez}, {\'A}. R. and {Lyubenova}, M. and {Marino}, R.~A. and {M{\'a}rmol-Queralt{\'o}}, E. and {M{\'a}rquez}, I. and {Masegosa}, J. and {Meidt}, S. and {Mendez-Abreu}, J. and {Monreal-Ibero}, A. and {Montijo}, C. and {Mour{\~a}o}, A.~M. and {Palacios-Navarro}, G. and {Papaderos}, P. and {Pasquali}, A. and {Peletier}, R. and {P{\'e}rez}, E. and {P{\'e}rez}, I. and {Quirrenbach}, A. and {Rela{\~n}o}, M. and {Rosales-Ortega}, F.~F. and {Roth}, M.~M. and {Ruiz-Lara}, T. and {S{\'a}nchez-Bl{\'a}zquez}, P. and {Sengupta}, C. and {Singh}, R. and {Stanishev}, V. and {Trager}, S.~C. and {Vazdekis}, A. and {Viironen}, K. and {Wild}, V. and {Zibetti}, S. and {Ziegler}, B.},
        title = "{CALIFA, the Calar Alto Legacy Integral Field Area survey. I. Survey presentation}",
      journal = {\aap},
     keywords = {techniques: spectroscopic, galaxies: active, galaxies: evolution, surveys, galaxies: ISM, galaxies: stellar content, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2012,
        month = feb,
       volume = {538},
          eid = {A8},
        pages = {A8},
          doi = {10.1051/0004-6361/201117353},
archivePrefix = {arXiv},
       eprint = {1111.0962},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...538A...8S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{bruzual03,
       author = {{Bruzual}, G. and {Charlot}, S.},
        title = "{Stellar population synthesis at the resolution of 2003}",
      journal = {\mnras},
     keywords = {stars: evolution, galaxies: evolution, galaxies: formation, galaxies: stellar content, Astrophysics},
         year = 2003,
        month = oct,
       volume = {344},
       number = {4},
        pages = {1000-1028},
          doi = {10.1046/j.1365-8711.2003.06897.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0309134},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003MNRAS.344.1000B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{willmer18,
       author = {{Willmer}, Christopher N.~A.},
        title = "{The Absolute Magnitude of the Sun in Several Filters}",
      journal = {\apjs},
     keywords = {astronomical databases: miscellaneous, catalogs, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = jun,
       volume = {236},
       number = {2},
          eid = {47},
        pages = {47},
          doi = {10.3847/1538-4365/aabfdf},
archivePrefix = {arXiv},
       eprint = {1804.07788},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..236...47W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}








@BOOK{gnuastrobook,
     author = {{Akhlaghi}, Mohammad},
      title = {GNU Astronomy Utilities (version 0.24), https://doi.org/10.5281/zenodo.17726900},
       year = 2025,
  publisher = {Free Software Foundation},
        doi = {10.5281/zenodo.17726900}
}










@ARTICLE{zahid17,
       author = {{Zahid}, H. Jabran and {Geller}, Margaret J.},
        title = "{Velocity Dispersion, Size, S{\'e}rsic Index, and D $_{ n }$4000: The Scaling of Stellar Mass with Dynamical Mass for Quiescent Galaxies}",
      journal = {\apj},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2017,
        month = may,
       volume = {841},
       number = {1},
          eid = {32},
        pages = {32},
          doi = {10.3847/1538-4357/aa7056},
archivePrefix = {arXiv},
       eprint = {1701.01350},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...841...32Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}









@ARTICLE{benitez14,
       author = {{Benitez}, N. and {Dupke}, R. and {Moles}, M. and {Sodre}, L. and {Cenarro}, J. and {Marin-Franch}, A. and {Taylor}, K. and {Cristobal}, D. and {Fernandez-Soto}, A. and {Mendes de Oliveira}, C. and {Cepa-Nogue}, J. and {Abramo}, L.~R. and {Alcaniz}, J.~S. and {Overzier}, R. and {Hernandez-Monteagudo}, C. and {Alfaro}, E.~J. and {Kanaan}, A. and {Carvano}, J.~M. and {Reis}, R.~R.~R. and {Martinez Gonzalez}, E. and {Ascaso}, B. and {Ballesteros}, F. and {Xavier}, H.~S. and {Varela}, J. and {Ederoclite}, A. and {Vazquez Ramio}, H. and {Broadhurst}, T. and {Cypriano}, E. and {Angulo}, R. and {Diego}, J.~M. and {Zandivarez}, A. and {Diaz}, E. and {Melchior}, P. and {Umetsu}, K. and {Spinelli}, P.~F. and {Zitrin}, A. and {Coe}, D. and {Yepes}, G. and {Vielva}, P. and {Sahni}, V. and {Marcos-Caballero}, A. and {Kitaura}, F. -S. and {Maroto}, A.~L. and {Masip}, M. and {Tsujikawa}, S. and {Carneiro}, S. and {Gonzalez Nuevo}, J. and {Carvalho}, G.~C. and {Reboucas}, M.~J. and {Carvalho}, J.~C. and {Abdalla}, E. and {Bernui}, A. and {Pigozzo}, C. and {Ferreira}, E.~G.~M. and {Chandrachani Devi}, N. and {Bengaly}, Jr., C.~A.~P. and {Campista}, M. and {Amorim}, A. and {Asari}, N.~V. and {Bongiovanni}, A. and {Bonoli}, S. and {Bruzual}, G. and {Cardiel}, N. and {Cava}, A. and {Cid Fernandes}, R. and {Coelho}, P. and {Cortesi}, A. and {Delgado}, R.~G. and {Diaz Garcia}, L. and {Espinosa}, J.~M.~R. and {Galliano}, E. and {Gonzalez-Serrano}, J.~I. and {Falcon-Barroso}, J. and {Fritz}, J. and {Fernandes}, C. and {Gorgas}, J. and {Hoyos}, C. and {Jimenez-Teja}, Y. and {Lopez-Aguerri}, J.~A. and {Lopez-San Juan}, C. and {Mateus}, A. and {Molino}, A. and {Novais}, P. and {OMill}, A. and {Oteo}, I. and {Perez-Gonzalez}, P.~G. and {Poggianti}, B. and {Proctor}, R. and {Ricciardelli}, E. and {Sanchez-Blazquez}, P. and {Storchi-Bergmann}, T. and {Telles}, E. and {Schoennell}, W. and {Trujillo}, N. and {Vazdekis}, A. and {Viironen}, K. and {Daflon}, S. and {Aparicio-Villegas}, T. and {Rocha}, D. and {Ribeiro}, T. and {Borges}, M. and {Martins}, S.~L. and {Marcolino}, W. and {Martinez-Delgado}, D. and {Perez-Torres}, M.~A. and {Siffert}, B.~B. and {Calvao}, M.~O. and {Sako}, M. and {Kessler}, R. and {Alvarez-Candal}, A. and {De Pra}, M. and {Roig}, F. and {Lazzaro}, D. and {Gorosabel}, J. and {Lopes de Oliveira}, R. and {Lima-Neto}, G.~B. and {Irwin}, J. and {Liu}, J.~F. and {Alvarez}, E. and {Balmes}, I. and {Chueca}, S. and {Costa-Duarte}, M.~V. and {da Costa}, A.~A. and {Dantas}, M.~L.~L. and {Diaz}, A.~Y. and {Fabregat}, J. and {Ferrari}, F. and {Gavela}, B. and {Gracia}, S.~G. and {Gruel}, N. and {Gutierrez}, J.~L.~L. and {Guzman}, R. and {Hernandez-Fernandez}, J.~D. and {Herranz}, D. and {Hurtado-Gil}, L. and {Jablonsky}, F. and {Laporte}, R. and {Le Tiran}, L.~L. and {Licandro}, J and {Lima}, M. and {Martin}, E. and {Martinez}, V. and {Montero}, J.~J.~C. and {Penteado}, P. and {Pereira}, C.~B. and {Peris}, V. and {Quilis}, V. and {Sanchez-Portal}, M. and {Soja}, A.~C. and {Solano}, E. and {Torra}, J. and {Valdivielso}, L.},
        title = "{J-PAS: The Javalambre-Physics of the Accelerated Universe Astrophysical Survey}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2014,
        month = mar,
          eid = {arXiv:1403.5237},
        pages = {arXiv:1403.5237},
          doi = {10.48550/arXiv.1403.5237},
archivePrefix = {arXiv},
       eprint = {1403.5237},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014arXiv1403.5237B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@INPROCEEDINGS{ds9,
       author = {{Joye}, W.~A. and {Mandel}, E.},
        title = "{New Features of SAOImage DS9}",
    booktitle = {Astronomical Data Analysis Software and Systems XII},
         year = 2003,
       editor = {{Payne}, H.~E. and {Jedrzejewski}, R.~I. and {Hook}, R.~N.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {295},
        month = jan,
        pages = {489},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ASPC..295..489J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}











@ARTICLE{elizabeth25,
       author = {{Sola}, Elisabeth and {Chemaly}, David and {Belokurov}, Vasily and {M{\"u}ller}, Oliver and {Ardern-Arentsen}, Anke and {Davies}, Elliot Y. and {Laguna-Miralles}, J{\'u}lia and {Myeong}, GyuChul and {Panagiotakis}, Konstantinos and {Zhang}, HanYuan and {Erkal}, Denis and {Koposov}, Sergey E. and {Lang}, Dustin and {Nibauer}, Jacob},
        title = "{STRRINGS: STReams in Residual Images of Nearby GalaxieS}",
      journal = {\mnras},
     keywords = {galaxies: interactions, galaxies: statistics, Astrophysics of Galaxies},
         year = 2025,
        month = nov,
       volume = {544},
       number = {1},
        pages = {735-763},
          doi = {10.1093/mnras/staf1647},
archivePrefix = {arXiv},
       eprint = {2508.02154},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2025MNRAS.544..735S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}









@ARTICLE{chabrier03,
       author = {{Chabrier}, Gilles},
        title = "{Galactic Stellar and Substellar Initial Mass Function}",
      journal = {\pasp},
     keywords = {Galaxies: Luminosity Function, Mass Function, Invited Reviews, Astrophysics},
         year = 2003,
        month = jul,
       volume = {115},
       number = {809},
        pages = {763-795},
          doi = {10.1086/376392},
archivePrefix = {arXiv},
       eprint = {astro-ph/0304382},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003PASP..115..763C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{salpeter55,
       author = {{Salpeter}, Edwin E.},
        title = "{The Luminosity Function and Stellar Evolution.}",
      journal = {\apj},
         year = 1955,
        month = jan,
       volume = {121},
        pages = {161},
          doi = {10.1086/145971},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1955ApJ...121..161S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{benito19,
       author = {{Garc{\'\i}a-Benito}, R. and {Gonz{\'a}lez Delgado}, R.~M. and {P{\'e}rez}, E. and {Cid Fernandes}, R. and {S{\'a}nchez}, S.~F. and {de Amorim}, A.~L.},
        title = "{Spatially resolved mass-to-light from the CALIFA survey. Mass-to-light ratio vs. color relations}",
      journal = {\aap},
     keywords = {techniques: spectroscopic, galaxies: star formation, galaxies: general, galaxies: evolution, galaxies: formation, surveys, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = jan,
       volume = {621},
          eid = {A120},
        pages = {A120},
          doi = {10.1051/0004-6361/201833993},
archivePrefix = {arXiv},
       eprint = {1811.08431},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...621A.120G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{alban23,
       author = {{Alb{\'a}n}, M. and {Wylezalek}, D.},
        title = "{Classifying the full SDSS-IV MaNGA Survey using optical diagnostic diagrams: Presentation of AGN catalogs in flexible apertures}",
      journal = {\aap},
     keywords = {catalogs, galaxies: active, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = jun,
       volume = {674},
          eid = {A85},
        pages = {A85},
          doi = {10.1051/0004-6361/202245437},
archivePrefix = {arXiv},
       eprint = {2302.08519},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...674A..85A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{fran25,
       author = {{Arizo-Borillo}, F.~D. and {Lopez-Sanjuan}, C. and {Pintos-Castro}, I. and {Fernandez-Ontiveros}, J.~A. and {Kuutma}, T. and {Lumbreras-Calle}, A. and {Hernan-Caballero}, A. and {Dominguez-Sanchez}, H. and {De Lucia}, G. and {Fontanot}, F. and {Diaz-Garcia}, L.~A. and {Vilchez}, J.~M. and {Rahna}, P.~T. and {Cenarro}, A.~J. and {Cristobal-Hornillos}, D. and {Hernandez-Monteagudo}, C. and {Marin-Franch}, A. and {Moles}, M. and {Varela}, J. and {Vazquez Ramio}, H. and {Alcaniz}, J. and {Dupke}, R.~A. and {Ederoclite}, A. and {Sodre}, Jr., L. and {Angulo}, R.~E.},
        title = "{J-PLUS: The stellar mass function of quiescent and star forming galaxies at 0.05 <= z <= 0.2}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics of Galaxies},
         year = 2025,
        month = sep,
          eid = {arXiv:2509.03404},
        pages = {arXiv:2509.03404},
          doi = {10.48550/arXiv.2509.03404},
archivePrefix = {arXiv},
       eprint = {2509.03404},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2025arXiv250903404A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}














@ARTICLE{Eskandarlou25,
       author = {{Eskandarlou}, Sepideh and {Akhlaghi}, Mohammad and {Knapen}, Johan H. and {L{\'o}pez-Sanjuan}, Carlos and {Infante-Sainz}, Ra{\'u}l and {Dom{\'\i}nguez S{\'a}nchez}, Helena and {Sharbaf}, Zahra and {V{\'a}zquez Rami{\'o}}, H{\'e}ctor and {Fern{\'a}ndez Ontiveros}, Juan Antonio and {I{\~n}iguez Garc{\'\i}a}, C{\'e}sar and {Civera Lorenzo}, Tamara and {Muniesa Gallardo}, David Jos{\'e} and {Coelho}, Paula R.~T. and {Ederoclite}, Alessandro and {Varela}, Jesus and {Jim{\'e}nez-Esteban}, Fran and {Cenarro}, Javier and {Mar{\'\i}n-Franch}, Antonio and {Dupke}, Renato A. and {Moles}, Mariano and {Hern{\'a}ndez-Monteagudo}, Carlos and {Rahna}, Payyasseri Thanduparackal and {Crist{\'o}bal-Hornillos}, David and {Alcaniz}, Jailson and {Sodr{\'e}}, Jr., Laerte and {Angulo}, Raul E.},
        title = "{J-PLUS: Turning off the bright stars}",
      journal = {\aap},
     keywords = {galaxies: halos, Instrumentation and Methods for Astrophysics, Astrophysics of Galaxies},
         year = 2026,
        month = jan,
       volume = {705},
          eid = {A67},
        pages = {A67},
          doi = {10.1051/0004-6361/202556547},
archivePrefix = {arXiv},
       eprint = {2510.12940},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2026A&A...705A..67E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
















@ARTICLE{Logro19,
       author = {{Logro{\~n}o-Garc{\'\i}a}, R. and {Vilella-Rojo}, G. and {L{\'o}pez-Sanjuan}, C. and {Varela}, J. and {Viironen}, K. and {Muniesa}, D.~J. and {Cenarro}, A.~J. and {Crist{\'o}bal-Hornillos}, D. and {Ederoclite}, A. and {Mar{\'\i}n-Franch}, A. and {Moles}, M. and {V{\'a}zquez Rami{\'o}}, H. and {Bonoli}, S. and {D{\'\i}az-Garc{\'\i}a}, L.~A. and {Orsi}, A. and {San Roman}, I. and {Akras}, S. and {Chies-Santos}, A.~L. and {Coelho}, P.~R.~T. and {Daflon}, S. and {Costa-Duarte}, M.~V. and {Dupke}, R. and {Galbany}, L. and {Gonz{\'a}lez Delgado}, R.~M. and {Hernandez-Jimenez}, J.~A. and {Lopes de Oliveira}, R. and {Mendes de Oliveira}, C. and {Oteo}, I. and {Gon{\c{c}}alves}, D.~R. and {S{\'a}nchez-Portal}, M. and {Schmidtobreick}, L. and {Sodr{\'e}}, L.},
        title = "{J-PLUS: Measuring H{\ensuremath{\alpha}} emission line fluxes in the nearby universe}",
      journal = {\aap},
     keywords = {methods: data analysis, techniques: photometric, galaxies: star formation, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = feb,
       volume = {622},
          eid = {A180},
        pages = {A180},
          doi = {10.1051/0004-6361/201732487},
archivePrefix = {arXiv},
       eprint = {1804.04039},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...622A.180L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

